Knowledge representation and diagnostic inference using Bayesian networks in the medical discourse

For the diagnostic inference under uncertainty Bayesian networks are investigated. The method is based on an adequate uniform representation of the necessary knowledge. This includes both generic and experience-based specific knowledge, which is stored in a knowledge base. For knowledge processing, a combination of the problem-solving methods of concept-based and case-based reasoning is used. Concept-based reasoning is used for the diagnosis, therapy and medication recommendation and evaluation of generic knowledge. Exceptions in the form of specific patient cases are processed by case-based reasoning. In addition, the use of Bayesian networks allows to deal with uncertainty, fuzziness and incompleteness. Thus, the valid general concepts can be issued according to their probability. To this end, various inference mechanisms are introduced and subsequently evaluated within the context of a developed prototype. Tests are employed to assess the classification of diagnoses by the network.

==> chapters/Anhang.tex <==
\chapter{Anhang}\label{chapter:attachment}
%\section{Dokumentation der beigelegten Software}
%Die im Rahmen der vorliegenden Arbeit implementierte Software ist als Projektmappe für Microsoft VisualStudio auf der beigelegten CD enthalten, zusammen mit der verwendeten Inferenzbibliothek Infer.NET. Eine detaillierte Dokumentation befindet sich ebenfalls auf der CD, sowohl im HTML-Format, als auch als PDF-Datei. Außerdem enthält die CD den \LaTeX-Quellcode der Arbeit selbst.

\section{Weitere Grafiken}
Die folgenden Grafiken enthalten die vollständige Darstellung der ermittelten Diagnosewahrscheinlichkeiten für alle Beispiele, die mit JTBP und VMP erzeugt wurden. Jeden von einem Algorithmus erzeugten Beispieldatensatz wurde pro Inferenzalgorithmus eine Grafik erstellt.

\begin{figure}[htbp!]
\makebox[\textwidth][c]{
    \tikzsetnextfilename{fulldataplot_JTBPsamples_EPinference}
    \begin{tikzpicture}
      \pgfplotsset{every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south}}
      \begin{axis}[
          xlabel=Erwartete Diagnose,
          ylabel=Wahrscheinlichkeit der Diagnose,
          legend style={font=\scriptsize,/tikz/every even column/.append style={column sep=0.28cm}},
          legend columns=5,
          xtick={100,300,500,700,900},
          xticklabels={BrainTumor,ClusterHeadache,MigraineWithAura,MigraineWithoutAura,TensionHeadache},
          x tick label style={font=\scriptsize},
          y tick label style={font=\scriptsize},
          width=1.05\linewidth, % Scale the plot to \linewidth
          minor xtick={200,400,600,800},
          minor ytick={0.2,0.4,0.6,0.8},
          grid=minor,
          grid style={dashed,gray!30},
          xmin=0, 
          xmax=1000,
          ymin=-1,
          ymax=1,
        ]
        \addplot[black, no markers, forget plot] coordinates {(0,0) (1000,0)};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x=x,y expr=\thisrow{BrainTumorF}*-1+0.04,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x=x,y expr=\thisrow{ClusterHeadacheF}*-1+0.03,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x=x,y expr=\thisrow{MigraineWithAuraF}*-1+0.02,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x=x,y expr=\thisrow{MigraineWithoutAuraF}*-1+0.01,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x=x,y expr=\thisrow{TensionHeadacheF}*-1,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x=x,y=TensionHeadacheT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x=x,y=MigraineWithoutAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x=x,y=MigraineWithAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x=x,y=ClusterHeadacheT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x=x,y=BrainTumorT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesEPInferredWithInf.csv};
          \legend{BrainTumor,ClusterHeadache,MigraineWithAura,MigraineWithoutAura,TensionHeadache}
      \end{axis}
    \end{tikzpicture}}
    \caption{Ergebnisse der Inferenz mit Expectation Propagation für die mit JTBP erzeugten Beispiele. Die Wahrscheinlichkeit für das Auftreten der erwarteten Diagnose gibt der Marker im positiven Bereich der y-Achse von 0 bis 1 an. Für die nicht erwarteten Diagnosen wird die Wahrscheinlichkeit für das Nicht-Eintreten dieser durch die Marker im negativen Bereich der y-Achse von -1 bis 0 angegeben. Welche Diagnose erwartet wurde, zeigt die Markierung an der X-Achse. Die negativen Werte wurden um bis zu 0,04 verschoben, um die Marker für jede Diagnose sichtbar zu machen.}\label{fig:results:full_plot:jtbp_samples:ep_inference}
\end{figure}

\begin{figure}[htbp!]
\makebox[\textwidth][c]{
    \tikzsetnextfilename{fulldataplot_JTBPsamples_JTBPinference}
    \begin{tikzpicture}
      \pgfplotsset{every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south}}
      \begin{axis}[
          xlabel=Erwartete Diagnose,
          ylabel=Wahrscheinlichkeit der Diagnose,
          legend style={font=\scriptsize,/tikz/every even column/.append style={column sep=0.28cm}},
          legend columns=5,
          xtick={100,300,500,700,900},
          xticklabels={BrainTumor,ClusterHeadache,MigraineWithAura,MigraineWithoutAura,TensionHeadache},
          x tick label style={font=\scriptsize},
          y tick label style={font=\scriptsize},
          width=1.05\linewidth, % Scale the plot to \linewidth
          minor xtick={200,400,600,800},
          minor ytick={0.2,0.4,0.6,0.8},
          grid=minor,
          grid style={dashed,gray!30},
          xmin=0, 
          xmax=1000,
          ymin=-1,
          ymax=1,
        ]
        \addplot[black, no markers, forget plot] coordinates {(0,0) (1000,0)};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{BrainTumorF}*-1+0.04,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{ClusterHeadacheF}*-1+0.03,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{MigraineWithAuraF}*-1+0.02,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{MigraineWithoutAuraF}*-1+0.01,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{TensionHeadacheF}*-1,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x expr=\thisrow{x}-2000,y=TensionHeadacheT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y=MigraineWithoutAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y=MigraineWithAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y=ClusterHeadacheT,col sep=comma]
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y=BrainTumorT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesJTBPInferredWithInf.csv};
          \legend{BrainTumor,ClusterHeadache,MigraineWithAura,MigraineWithoutAura,TensionHeadache}
      \end{axis}
    \end{tikzpicture}}
    \caption{Ergebnisse der Inferenz mit Join Tree Belief Propagation für die mit JTBP erzeugten Beispiele. Die Wahrscheinlichkeit für das Auftreten der erwarteten Diagnose gibt der Marker im positiven Bereich der y-Achse von 0 bis 1 an. Für die nicht erwarteten Diagnosen wird die Wahrscheinlichkeit für das Nicht-Eintreten dieser durch die Marker im negativen Bereich der y-Achse von -1 bis 0 angegeben. Welche Diagnose erwartet wurde, zeigt die Markierung an der X-Achse.Die negativen Werte wurden um bis zu 0,04 verschoben, um die Marker für jede Diagnose sichtbar zu machen.}\label{fig:results:full_plot:jtbp_samples:jtbp_inference}
\end{figure}

\begin{figure}[htbp!]
\makebox[\textwidth][c]{
    \tikzsetnextfilename{fulldataplot_JTBPsamples_VMPinference}
    \begin{tikzpicture}
      \pgfplotsset{every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south}}
      \begin{axis}[
          xlabel=Erwartete Diagnose,
          ylabel=Wahrscheinlichkeit der Diagnose,
          legend style={font=\scriptsize,/tikz/every even column/.append style={column sep=0.28cm}},
          legend columns=5,
          xtick={100,300,500,700,900},
          xticklabels={BrainTumor,ClusterHeadache,MigraineWithAura,MigraineWithoutAura,TensionHeadache},
          x tick label style={font=\scriptsize},
          y tick label style={font=\scriptsize},
          width=1.05\linewidth, % Scale the plot to \linewidth
          minor xtick={200,400,600,800},
          minor ytick={0.2,0.4,0.6,0.8},
          grid=minor,
          grid style={dashed,gray!30},
          xmin=0, 
          xmax=1000,
          ymin=-1,
          ymax=1,
        ]
        \addplot[black, no markers, forget plot] coordinates {(0,0) (1000,0)};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{BrainTumorF}*-1+0.04,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{ClusterHeadacheF}*-1+0.03,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{MigraineWithAuraF}*-1+0.02,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{MigraineWithoutAuraF}*-1+0.01,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{TensionHeadacheF}*-1,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x expr=\thisrow{x}-1000,y=TensionHeadacheT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y=MigraineWithoutAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y=MigraineWithAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y=BrainTumorT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y=ClusterHeadacheT,col sep=comma]
          {\mainpath/chapters/tables/JoinedResultProbsJTBPSamplesVMPInferredWithInf.csv};
          \legend{BrainTumor,ClusterHeadache,MigraineWithAura,MigraineWithoutAura,TensionHeadache}
      \end{axis}
    \end{tikzpicture}}
    \caption{Ergebnisse der Inferenz mit Variational Message Passing für die mit JTBP erzeugten Beispiele. Die Wahrscheinlichkeit für das Auftreten der erwarteten Diagnose gibt der Marker im positiven Bereich der y-Achse von 0 bis 1 an. Für die nicht erwarteten Diagnosen wird die Wahrscheinlichkeit für das Nicht-Eintreten dieser durch die Marker im negativen Bereich der y-Achse von -1 bis 0 angegeben. Welche Diagnose erwartet wurde, zeigt die Markierung an der X-Achse.Die negativen Werte wurden um bis zu 0,04 verschoben, um die Marker für jede Diagnose sichtbar zu machen.}\label{fig:results:full_plot:jtbp_samples:vmp_inference}
\end{figure}
\begin{figure}[htbp!]
\makebox[\textwidth][c]{
    \tikzsetnextfilename{fulldataplot_VMPsamples_EPinference}
    \begin{tikzpicture}
      \pgfplotsset{every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south}}
      \begin{axis}[
          xlabel=Erwartete Diagnose,
          ylabel=Wahrscheinlichkeit der Diagnose,
          legend style={font=\scriptsize,/tikz/every even column/.append style={column sep=0.28cm}},
          legend columns=5,
          xtick={100,300,500,700,900},
          xticklabels={BrainTumor,MigraineWithAura,MigraineWithoutAura,TensionHeadache,ClusterHeadache},
          x tick label style={font=\scriptsize},
          y tick label style={font=\scriptsize},
          width=1.05\linewidth, % Scale the plot to \linewidth
          minor xtick={200,400,600,800},
          minor ytick={0.2,0.4,0.6,0.8},
          grid=minor,
          grid style={dashed,gray!30},
          xmin=0, 
          xmax=1000,
          ymin=-1,
          ymax=1,
        ]
        \addplot[black, no markers, forget plot] coordinates {(0,0) (1000,0)};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x=x,y expr=\thisrow{BrainTumorF}*-1+0.04,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x=x,y expr=\thisrow{MigraineWithAuraF}*-1+0.03,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x=x,y expr=\thisrow{MigraineWithoutAuraF}*-1+0.02,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x=x,y expr=\thisrow{TensionHeadacheF}*-1+0.01,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x=x,y expr=\thisrow{ClusterHeadacheF}*-1,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x=x,y=ClusterHeadacheT,col sep=comma] {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x=x,y=TensionHeadacheT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x=x,y=MigraineWithoutAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x=x,y=MigraineWithAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x=x,y=BrainTumorT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesEPInferredWithInf.csv};
          \legend{BrainTumor,MigraineWithAura,MigraineWithoutAura,TensionHeadache,ClusterHeadache}
      \end{axis}
    \end{tikzpicture}}
    \caption{Ergebnisse der Inferenz mit Expectation Propagation für die mit VMP erzeugten Beispiele. Die Wahrscheinlichkeit für das Auftreten der erwarteten Diagnose gibt der Marker im positiven Bereich der y-Achse von 0 bis 1 an. Für die nicht erwarteten Diagnosen wird die Wahrscheinlichkeit für das Nicht-Eintreten dieser durch die Marker im negativen Bereich der y-Achse von -1 bis 0 angegeben. Welche Diagnose erwartet wurde, zeigt die Markierung an der X-Achse. Die negativen Werte wurden um bis zu 0,04 verschoben, um die Marker für jede Diagnose sichtbar zu machen.}\label{fig:results:full_plot:vmp_samples:ep_inference}
\end{figure}

\begin{figure}[htbp!]
\makebox[\textwidth][c]{
    \tikzsetnextfilename{fulldataplot_VMPsamples_JTBPinference}
    \begin{tikzpicture}
      \pgfplotsset{every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south}}
      \begin{axis}[
          xlabel=Erwartete Diagnose,
          ylabel=Wahrscheinlichkeit der Diagnose,
          legend style={font=\scriptsize,/tikz/every even column/.append style={column sep=0.28cm}},
          legend columns=5,
          xtick={100,300,500,700,900},
          xticklabels={BrainTumor,MigraineWithAura,MigraineWithoutAura,TensionHeadache,ClusterHeadache},
          x tick label style={font=\scriptsize},
          y tick label style={font=\scriptsize},
          width=1.05\linewidth, % Scale the plot to \linewidth
          minor xtick={200,400,600,800},
          minor ytick={0.2,0.4,0.6,0.8},
          grid=minor,
          grid style={dashed,gray!30},
          xmin=0, 
          xmax=1000,
          ymin=-1,
          ymax=1,
        ]
        \addplot[black, no markers, forget plot] coordinates {(0,0) (1000,0)};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{BrainTumorF}*-1+0.04,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{MigraineWithAuraF}*-1+0.03,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{MigraineWithoutAuraF}*-1+0.02,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{TensionHeadacheF}*-1+0.01,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y expr=\thisrow{ClusterHeadacheF}*-1,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y=ClusterHeadacheT,col sep=comma]
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x expr=\thisrow{x}-2000,y=TensionHeadacheT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y=MigraineWithoutAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y=MigraineWithAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-2000,y=BrainTumorT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesJTBPInferredWithInf.csv};
          \legend{BrainTumor,MigraineWithAura,MigraineWithoutAura,TensionHeadache,ClusterHeadache}
      \end{axis}
    \end{tikzpicture}}
    \caption{Ergebnisse der Inferenz mit Join Tree Belief Propagation für die mit VMP erzeugten Beispiele. Die Wahrscheinlichkeit für das Auftreten der erwarteten Diagnose gibt der Marker im positiven Bereich der y-Achse von 0 bis 1 an. Für die nicht erwarteten Diagnosen wird die Wahrscheinlichkeit für das Nicht-Eintreten dieser durch die Marker im negativen Bereich der y-Achse von -1 bis 0 angegeben. Welche Diagnose erwartet wurde, zeigt die Markierung an der X-Achse.Die negativen Werte wurden um bis zu 0,04 verschoben, um die Marker für jede Diagnose sichtbar zu machen.}\label{fig:results:full_plot:vmp_samples:jtbp_inference}
\end{figure}

\begin{figure}[htbp!]
\makebox[\textwidth][c]{
    \tikzsetnextfilename{fulldataplot_VMPsamples_VMPinference}
    \begin{tikzpicture}
      \pgfplotsset{every axis legend/.append style={
        at={(0.5,1.03)},
        anchor=south}}
      \begin{axis}[
          xlabel=Erwartete Diagnose,
          ylabel=Wahrscheinlichkeit der Diagnose,
          legend style={font=\scriptsize,/tikz/every even column/.append style={column sep=0.28cm}},
          legend columns=5,
          xtick={100,300,500,700,900},
          xticklabels={BrainTumor,MigraineWithAura,MigraineWithoutAura,TensionHeadache,ClusterHeadache},
          x tick label style={font=\scriptsize},
          y tick label style={font=\scriptsize},
          width=1.05\linewidth, % Scale the plot to \linewidth
          minor xtick={200,400,600,800},
          minor ytick={0.2,0.4,0.6,0.8},
          grid=minor,
          grid style={dashed,gray!30},
          xmin=0, 
          xmax=1000,
          ymin=-1,
          ymax=1,
        ]
        \addplot[black, no markers, forget plot] coordinates {(0,0) (1000,0)};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{BrainTumorF}*-1+0.04,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{MigraineWithAuraF}*-1+0.03,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{MigraineWithoutAuraF}*-1+0.02,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{TensionHeadacheF}*-1+0.01,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y expr=\thisrow{ClusterHeadacheF}*-1,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
        \addplot[blue, only marks, mark=square*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y=ClusterHeadacheT,col sep=comma]
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
        \addplot[purple, only marks, mark=triangle*, mark options={mark size=1,rotate=180}] 
          table[x expr=\thisrow{x}-1000,y=TensionHeadacheT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
        \addplot[orange, only marks, mark=diamond*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y=MigraineWithoutAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
        \addplot[green, only marks, mark=triangle*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y=MigraineWithAuraT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
        \addplot[red, only marks, mark=*, mark options={mark size=1}] 
          table[x expr=\thisrow{x}-1000,y=BrainTumorT,col sep=comma] 
          {\mainpath/chapters/tables/JoinedResultProbsVMPSamplesVMPInferredWithInf.csv};
          \legend{BrainTumor,MigraineWithAura,MigraineWithoutAura,TensionHeadache,ClusterHeadache}
      \end{axis}
    \end{tikzpicture}}
    \caption{Ergebnisse der Inferenz mit Variational Message Passing für die mit VMP erzeugten Beispiele. Die Wahrscheinlichkeit für das Auftreten der erwarteten Diagnose gibt der Marker im positiven Bereich der y-Achse von 0 bis 1 an. Für die nicht erwarteten Diagnosen wird die Wahrscheinlichkeit für das Nicht-Eintreten dieser durch die Marker im negativen Bereich der y-Achse von -1 bis 0 angegeben. Welche Diagnose erwartet wurde, zeigt die Markierung an der X-Achse.Die negativen Werte wurden um bis zu 0,04 verschoben, um die Marker für jede Diagnose sichtbar zu machen.}\label{fig:results:full_plot:vmp_samples:vmp_inference}
\end{figure}
\clearpage

%\section{Weitere Tabellen}
%Auf den folgenden Seiten sind Wahrscheinlichkeitsverteilungen der einzelnen Merkmale für jede Diagnose aufgeführt (Tabelle \ref{tab:observable_distributions}), die den mit EP erzeugten Beispielen zugrunde liegen, sowie die Wahrscheinlichkeiten der einzelnen Diagnosen für alle Beispiele, die bei der Inferenz der mit EP falsch klassifiziert wurden (wahrscheinlichste Diagnose entspricht nicht der Diagnose, die der Erzeugung der Merkmalswerte des Beispieles zugrunde lag). Auf die Darstellung der äquivalenten Tabellen für die mit JTBP und VMP erzeugten Beispiele wurde verzichtet, da sie keine statistisch signifikanten Unterschiede zu den folgenden Tabellen aufweisen. Die zugrundeliegenden Datenbanken sind jedoch vollständig auf der beigelegten CD enthalten.
%\clearpage
%\input{\mainpath/chapters/tables/RoundedSymptomProbabilityComparisonByAlgorithm.tex}
%
%\clearpage
%\input{\mainpath/chapters/tables/WrongClassificationProbsPretty_EP.tex}
%\clearpage


==> chapters/Ausblick.tex <==
\chapter{Zusammenfassung und Ausblick}
\textcolor{red}{überarbeiten} \\

%Das Ziel der vorliegenden Arbeit war, einen prototypischen Agenten zu bauen, welcher ein Bayessches Netz in einem externen Textformat verarbeiten und darauf Abfragen durchführen kann. Dieses Ziel wurde erreicht. Mit der Implementierung in der Programmiersprache C\# unter Verwendung von Infer.NET wurde auch die Anforderung erfüllt, eine leichte Integrierbarkeit in den bestehenden Quellcode der iSuite zu gewährleisten. Mit PGMX wurde ein flexibles Format für die externe Repräsentation gefunden, welches insbesondere die Modellierung von kompakten Knotenbeziehungen wie \textit{Noisy-OR} und \textit{Noisy-MAX} ermöglicht. Das prototypische Kopfschmerznetz aus \cite{beleg} wurde in dieses Format überführt und die vorgelegte Implementierung eines Agenten ist in der Lage, dieses Netz in ein Infer.NET-Modell zu überführen und Abfragen an dieses Netz mit Hilfe von Infer.NET zu beantworten.

Um die Qualität eines Bayesschen Netzes und eines Inferenzalgorithmus zu bewerten, wurde ein Werkzeug geschaffen, um Beispielabfragen für ein Netz zu generieren und diese mithilfe des Netzes auszuwerten. Das Werkzeug wurde genutzt, um die von Infer.NET zur Verfügung gestellten Algorithmen \textit{Expectation Propagation} und \textit{Variational Message Passing} zu analysieren und mit dem \textit{Join Tree Belief Propagation} zu vergleichen. Ebenso wurde das Bayessche Netz aus Abbildung \ref{fig:full_network} modelliert und festgestellt, dass es für die modellierte Domäne der Kopfschmerzdiagnostik sehr gute Ergebnisse liefert. Zudem wurde gezeigt, dass EP als Inferenzalgorithmus für diese Domäne geeigneter ist als VMP und eine ebenso hohe Inferenzqualität hat, wie JTBP.

Um die Domäne der Schmerzdiagnostik vollständig abzudecken, ist die Konstruktion weiterer Bayesscher Netze notwendig. Dabei ist eine Zusammenarbeit mit Fachleuten aus der Schmerzdiagnostik unabdingbar, denn für die Modellierung stehen in der Regel nur unvollständige und ungenaue Statistiken zur Verfügung. In \cite{Nikovski_2000_3154_2} werden geeignete Konstruktionsmethoden beschrieben, die diese Probleme adressieren und in einem iterativen Entwurfsprozess angewendet werden können. Der im Rahmen dieser Arbeit entwickelte Beispielgenerator kann dabei als wichtiges Hilfsmittel dienen. Noch zu entwickelnde graphische Werkzeuge könnten die Netzkonstruktion deutlich erleichtern \textendash das verwendete Format zur externen Netzrepräsentation bietet die Möglichkeit, Daten zu speichern, die für einen graphischen Editor notwendig sind (beispielsweise die Koordinaten eines Netzknotens). \cite{pittir10084} arbeitet wichtige Aspekte heraus, die bei der Entwicklung eines solchen Editors berücksichtigt werden müssen und liefert gute Vorschläge für die praktische Umsetzung.

Um die konstruierten Bayesschen Netze in diagnostischen Systemen nutzen zu können, muss der entwickelte Agent in das jeweilige System integriert und mit der bestehenden Schnittstelle zur Abfrage von Anamnesedaten verbunden werden. Dabei können die Informationen eines Bayesschen Netzes auf eine Weise genutzt werden, die über die reine Ermittlung von Diagnosewahrscheinlichkeiten zu einer gegebenen Anamnese hinausgeht. Zum Beispiel können die A-Posteriori-Verteilungen von Symptom-Merkmalen, wie sie auch zur Generierung der Beispielabfragen verwendet wurden, dazu dienen, ein Ähnlichkeitsmaß für Diagnosen zu definieren. Mit der Bestimmung eines minimalen Abstandes könnten dann Differentialdiagnosen zur berechneten wahrscheinlichsten Diagnose ermittelt werden und mit einem maximalen Abstand differentialdiagnostisch besonders kritische Merkmale und Symptome zwischen diesen zwei Diagnosen. Beides könnte dem Arzt zusammen mit den Diagnosewahrscheinlichkeiten präsentiert werden und ihn darauf hinweisen, auf diese Symptome ein besonderes Augenmerk zu legen. Welches Abstandsmaß für einen solchen Anwendungsfall geeignet wäre, müsste noch untersucht werden.

Für all dies wurde mit den Ergebnissen der vorliegenden Arbeit ein wichtiger Grundstein gelegt, der sowohl im Rahmen der allgemeinen praktischen Arbeit mit Bayesschen Netzen als auch für deren spezielle Verwendung im medizinischen Anwendungskontext vielversprechende Entwicklungen ermöglicht.


==> chapters/Theorie.tex <==
\chapter{Theoretische Grundlagen}
\label{chapter:theory}

\section{Definition und Konstruktion Bayesscher Netze}
\label{chapter:theory:sec:bn_definition}
Im medizinischen Diskursbereich müssen häufig Entscheidungen getroffen werden, die auf unsicherem Wissen basieren. Dieses Wissen kann durch eine n-dimensionale Zufallsvariable $X_1 \dots X_n$ repräsentiert werden, deren Werte voneinander abhängig sein können. Bayessche Netze dienen zur Konstruktion einer solchen hochdimensionalen Wahrscheinlichkeitsverteilung. Sie basieren auf lokalen probabilistischen Regeln, die statistische Abhängigkeiten zwischen Merkmalen berücksichtigen und sich damit eng an einer kausalen Modellierung der Welt orientieren. Deshalb lassen sich mit Bayesschen Netzen komplexe Problemstellungen mit einer verhältnismäßig geringen Zahl bedingter Wahrscheinlichkeiten modellieren.

\begin{Def}[Bayessches Netz]
Ein Bayessches Netz ist ein Probabilistisches Graphisches Modell (PGM), das der Abbildung unscharfen Wissens in einer geschlossenen Domain dient. Es besteht aus einem Graphen und lokalen Wahrscheinlichkeitsverteilungen. Es gelten folgende Eigenschaften:
\begin{itemize}
 \item Die Beziehungen zwischen den Knoten des Graphen sind \tbf{gerichtet} und der Graph ist \tbf{zyklenfrei} (DAG).
 \item Jede Kante beschreibt eine Eltern-Kind-Beziehung zwischen zwei Knoten. Der Ausgangsknoten heißt \tbf{Elternknoten}, der Zielknoten heißt \tbf{Kindknoten}.
 \item Jeder Knoten repräsentiert eine Zufallsvariable $X$ mit einem Wertebereich, der diskret oder stetig sein kann.\footnote{In der medizinischen Diagnostik sind die meisten Knoten nur binär.} Mit $\prb{\Pi}_X$ bezeichnen wir die Menge der Elternknoten, mit $\prb{\pi}_X$ ihre Instanziierungen. 
 \item Jeder Knoten enthält eine \tbf{lokale Wahrscheinlichkeitsverteilung}. Für Kindknoten ist diese Wahrscheinlichkeitsverteilung eine bedingte Wahrscheinlichkeitsverteilung $\prb{P}(X|\prb{\Pi}_{X})$, welche den Effekt der Elternknoten $\prb{\Pi}_{X}$ auf den Knoten $X$ quantifiziert. Für Knoten mit $\prb{\Pi}_X = \emptyset$ gelten unbedingte A-priori-Verteilungen $\prb{P}(X)$.
\end{itemize}
\end{Def}

Die vollständige gemeinsame Verteilung, auch \tbf{Verbunddichte} genannt, enthält das gesamte unsichere Wissen über eine Domäne. Ein Bayessches Netz lässt sich als Darstellung einer solchen Verteilung auffassen. 

\begin{Def}[Verbunddichte]
Sei $P(x_1, ..., x_n)$ ein generischer Eintrag in der Wahrscheinlichkeitstabelle, wobei $x_1$ bis $x_n$ konkrete Wertzuweisungen zu den einzelnen Knoten sind. Die Wahrscheinlichkeit dieser Wertzuweisung lässt sich als Produkt der bedingten Wahrscheinlichkeiten der einzelnen Knoten wie folgt ausdrücken:
\begin{align}
\label{Verbunddichte}
P(x_1, ..., x_n)=\prod_{i=1}^{n}P(x_i|\prb{\pi}_i).
\end{align}
$\prb{\pi}_i$ sind die konkreten Instanziierungen der Elternknoten $\prb{\Pi}_i$, welche in den Verteilungen $x_1, ..., x_n$ erscheinen.
\end{Def}

Für die Konstruktion eines Bayesschen Netzes, das die Domäne möglichst gut repräsentiert, werden bedingte Unabhängigkeiten benötigt, welche von \eqref{Verbunddichte} impliziert werden. Mit der Produktregel lässt sich \eqref{Verbunddichte} auch wie folgt schreiben:
\begin{align*}
P(x_1,..., x_n)=P(x_n|x_{n-1},...,x_1)P(x_{n-1},...,x_1).
\end{align*}
Ein wiederholtes Anwenden der Produktregel, auch Kettenregel genannt, ergibt folgendes großes Produkt:
\begin{align*}
P(x_1,..., x_n)&=P(x_n|x_{n-1},...,x_1)P(x_{n-1}|x_{n-2},...,x_1)...P(x_2|x_1)P(x_1)\\
&=\prod_{i=1}^{n}P(x_i|x_{i-1},...,x_1).
\end{align*}
Verglichen mit \eqref{Verbunddichte} gilt somit für jede Variable $X_i$ des Netzes und ihre Elternknoten $\prb{\Pi}_i$:
\begin{align}
\label{Nummerierung}
\prb{P}(X_i|X_{i-1},...,X_1)=\prb{P}(X_i|\prb{\Pi}_i)
\end{align}
unter der Voraussetzung $\prb{\Pi}_i\subseteq\{X_{i-1},..., X_1\}$.
Aus Gleichung \eqref{Nummerierung} geht hervor, dass ein Bayessches Netz eine Domäne nur dann korrekt repräsentiert, wenn ein Knoten $X_i$ bei bekannten Eltern $\prb{\Pi}_i$ bedingt unabhängig von seinen restlichen Vorgängern in der Knotenreihenfolge ist.

Folgender Algorithmus erzeugt ein Netz, welches diese Bedingungen erfüllt.

\begin{Alg}[Konstruktion eines Bayesschen Netzes]
\begin{enumerate}
 \item \textit{Knoten}: Bestimme die Menge von Zufallsvariablen $X_i$, welche für die Domäne relevant sind. Um eine möglichst kompakte Netzstruktur zu erreichen, sortiere sie in der Reihenfolge, dass Ursachen vor Wirkungen erscheinen. Wir erhalten $\{X_1,\dots, X_n\}$.
 \item \textit{Kanten}: Führe für $i=1$ bis $n$ aus:
 \begin{itemize}
  \item Wähle aus der Menge $\{X_1, ..., X_{i-1}\}$ eine minimale Teilmenge von Eltern $\prb{\Pi}_i$, welche die Gleichung \eqref{Nummerierung} erfüllt.
  \item Füge für jedes Element aus $\prb{\Pi}_i$ eine gerichtete Kante vom Elternknoten zum Knoten $X_i$ ein.
  \item Definiere die bedingte Wahrscheinlichkeitsverteilung $\prb{P}(X_i|\prb{\Pi}_i)$.
 \end{itemize}
\end{enumerate}
\end{Alg}

Mit anderen Worten: $\prb{\Pi}_i$ soll alle Knoten aus $\{X_1,\dots,X_{i-1}\}$ enthalten, die $X_i$ direkt beeinflussen.

Der beschriebene Algorithmus garantiert Azyklizität, da jeder Knoten nur mit Knoten verbunden ist, die in der nach Kausalität sortierten Knotenmenge vor ihm liegen.

Die nachfolgende Abbildung \ref{Karzinomnetz} zeigt ein Beispiel eines Bayesschen Netzes in der Medizin zur Berechnung der Wahrscheinlichkeit eines Schlaganfalls und Herzinfarkts. Diabetes Mellitus $D$ hat möglicherweise Arteriosklerose (Gefäßverkalkung) $A$ und Hypertonie (Bluthochdruck) $H$ zur Folge, welche wiederum bewirken können, dass der Patient einen Herzinfarkt $I$ hat. Außerdem kann Arteriosklerose zu einem Schlaganfall $S$ führen.

\begin{figure}[ht!]
	\centering
	{\renewcommand{\arraystretch}{1.3}
		\begin{tikzpicture}[every label/.style={font=\small}]
		\tikzstyle{vertex}=[circle, draw, font=\small, inner sep=0pt, minimum size=25pt]
		\tikzstyle{phantom}=[vertex,draw=none]
		
		\node[vertex] (D) at (0,0) {$D$};
		\node[above=0.5 of D] (DA){
			\begin{tabular}{|c|l|l|}
			\hline
			\multicolumn{3}{|c|}{Diabetes mellitus $D$} \\ \hline
			$P(D)$ & $d$ & $\neg d$ \\ \hline
			& 0,2 & 0,8 \\ \hline
			\end{tabular}
		};
		\node[vertex, below left=1.5 of D] (A) {$A$};
		\node[above left=0.5 of A] (AA) {
			\begin{tabular}{|r|l|l|}
			\hline
			\multicolumn{3}{|c|}{Arteriosklerose $A$} \\ \hline
			$P(A|D)$ & $a$  & $\neg a$ \\ \hline
			$d$      & 0,2  & 0,8      \\ 
			$\neg d$ & 0,05 & 0,95     \\ \hline
			\end{tabular}
		};
		\node[vertex, below right=1.5 of D] (H) {$H$};
		\node[above right=0.5 of H] (HA) {
			\begin{tabular}{|r|l|l|}
			\hline
			\multicolumn{3}{|c|}{Hypteronie $H$} \\ \hline
			$P(H|D)$ & $h$ & $\neg h$ \\ \hline
			$d$      & 0,8 & 0,2      \\ 
			$\neg d$ & 0,2 & 0,8      \\ \hline
			\end{tabular}
		};
		\node[vertex, below=1.5 of H] (I) {$C$};
		\node[right=0.5 of I] (IA) {
			\begin{tabular}{|r r|l|l|}
			\hline
			\multicolumn{4}{|c|}{Herzinfarkt $I$} \\ \hline
			\multicolumn{2}{|c|}{$P(I|A,H)$}
			& $h$  & $\neg h$ \\ \hline
			$a$,     & $h$     & 0,8  & 0,2      \\ 
			$a$,     &$\neg h$ & 0,8  & 0,2      \\
			$\neg a$,&$ h$     & 0,8  & 0,2      \\ 
			$\neg a$,&$\neg h$ & 0,05 & 0,95     \\ \hline
			\end{tabular}
		};
		\node[vertex, below=1.5 of A] (S) {$S$};
		\node[left=0.5 of S] (SA) {
			\begin{tabular}{|r|l|l|}
			\hline
			\multicolumn{3}{|c|}{Schlaganfall $S$} \\ \hline
			$P(S|A)$ & $h$ & $\neg h$ \\ \hline
			$d$      & 0,8 & 0,2      \\ 
			$\neg d$ & 0,6 & 0,4      \\ \hline
			\end{tabular}
		};
		\path
		(D) edge[e] (A)
		(D) edge[e] (H)
		(A) edge[e] (I)
		(H) edge[e] (I)
		(A) edge[e] (S)
		;
		\end{tikzpicture}}
	\caption{Beispiel eines einfachen Bayesschen Netzes in der Medizin}
	\label{Karzinomnetz}
\end{figure}

%\section{Struktureigenschaften}

%\paragraph{Lokale Strukturierung und Kompaktheit}
%Bayessche Netze gehören zur Klasse der lokal strukturierten Systeme. Ein lokal strukturiertes System besteht aus Unterkomponenten, wobei jede Komponente nur mit einer begrenzten Anzahl anderer Komponenten interagiert, unabhängig von der Gesamtzahl der Komponenten. Ein solches System weist deshalb meist ein lineares statt ein exponentielles Komplexitätswachstum auf. 
%
%Übertragen auf Bayessche Netze heißt das, dass jede Zufallsvariable nur von einer begrenzten Anzahl anderer Zufallsvariablen direkt beeinflusst wird. Sei diese Anzahl mit der Konstante $k$ bezeichnet und man betrachte ein Netz mit $n$ boolschen Variablen. Da für die Angabe der bedingten Wahrscheinlichkeiten pro Variable maximal $2^k$ Zahlen benötigt werden, sind nur $n2^k$ Zahlen für die Spezifikation des vollständigen Netzes nötig, während die vollständige gemeinsame Verteilung jedoch $2^n$ Zahlen enthält. Je größer also die Anzahl der Knoten ist, desto drastischer ist dieser Unterschied. Somit sind Bayessche Netze eine besonders kompakte Repräsentation einer vollständigen gemeinsamen Verteilung.
%
%\paragraph{Bedingte Unabhängigkeit}
%Eine Unabhängigkeitsaussage der Form $X$ und $Y$ sind unabhängig bei bekanntem $Z$ heißt, dass für alle Kombinationen der Werte $x$, $y$ und $z$ folgende Gleichung gilt:
%$$\prb{P}(\prb{x}|\prb{z})=\prb{P}(\prb{x}|\prb{yz}).$$
%Anders formuliert: Ist $z$ bekannt, wird die Kenntnis von $y$ die Vorstellung von $x$ nicht beeinflussen.
%
%Die Graphstruktur des Netzes kodiert bedingte Unabhängigkeitsaussagen. Zwei und mehr Unabhängigkeitsaussagen können eine weitere Unabhängigkeitsaussage implizieren. Die hierbei geltenden Regeln sind als Graphoid-Axiome definiert. Die sogenannte d-Separation ist eine graphentheoretische Relation, die alle diese ableitbaren Unabhängigkeiten abdeckt. $Z$ d-separiert $X$ und $Y$ in einem DAG, wenn innerhalb des Netzes $X$ und $Y$ bei bekanntem $Z$ unabhängig bezüglich der Graphoid-Axiome sind. 

\section{Repräsentation bedingter Verteilungen}
Die bedingten Verteilungen können als Wahrheitswertetabelle notiert werden. Dies wird aber schon bei wenigen Parametern ineffizient, da Kombinationsmöglichkeiten aus Zuständen von Eltern- und Kindknoten und damit die Anzahl der Zeilen einer Wahrheitswertetabelle exponentiell steigt. Gefragt sind kompaktere Möglichkeiten zur Darstellung lokaler Beziehungen zwischen den Zufallsvariablen. Etabliert hat sich ein Katalog aus kanonischen Wahrscheinlichkeitsmodellen \cite{Diez00canonicalprobabilistic}, welche mit wenigen Parameter größere bedingte Verteilungen modellieren können. Im Folgenden werden die Beziehungen erläutert, welche zur Modellierung des prototypischen Netzes verwendet wurden und vom implementierten Agenten verarbeitet werden können. Eine Erweiterung des Agenten um weitere kanonische Modelle ist mit überschaubarem Aufwand möglich.

\subsection{Vollständige bedingte Wahrscheinlichkeitstabelle}
Der einfachste Fall ist eine vollständig ausgefüllte bedingte Wahrscheinlichkeitstabelle (BWT). Für jede Kombination von möglichen Zuständen eines Kindknotens und seiner Elternknoten muss eine Wahrscheinlichkeit gefunden werden. Diese Zustandskombination bildet zusammen mit der Wahrscheinlichkeit eine Zeile der Tabelle. Somit wird die direkte Notation einer solchen Tabelle schon bei wenigen Elternknoten unpraktikabel. 
%Beispiele für BWTs zeigt Abbildung \ref{Karzinomnetz} (Seite \pageref{Karzinomnetz}) .

Kanonische Wahrscheinlichkeitsmodelle stellen eine Möglichkeit dar, eine bedingte Wahrscheinlichkeitsverteilung mit wenigen Parametern anzugeben. Mittels der jeweiligen Berechnungsformel der kanonischen Verteilung wird aus den Parametern eine vollständige bedingte Wahrscheinlichkeitstabelle konstruiert.

\subsection{Deterministischer Knoten}
\label{sec:deterministic_var}
Der einfachste Fall einer Beziehung zwischen Eltern- und Kindknoten ist eine deterministische, also keinerlei Unsicherheit enthaltende Relation. Der Wert des Kindknotens wird durch eine Funktion bestimmt, die die Werte der Elternknoten als Parameter entgegennimmt. 

\begin{Def}[Bedingte Wahrscheinlichkeitsverteilung]
Die bedingte Wahrscheinlichkeit ergibt sich wie folgt:
$$P(y|\prb x) = \begin{cases}
 1 & \mbox{wenn } y = f(x) \\
 0 & \mbox{sonst.}
\end{cases}$$
\end{Def}

Eine Liste gängiger Funktionen ist in Tabelle \ref{Deterministische Funktionen} aufgeführt.
\begin{table}[h]
 \centering
 \captionsetup{width=0.8\textwidth}
 \begin{tabular}{|c|c|ll|}
 \hline
 Funktionstyp & Variablentyp & \multicolumn{1}{|c}{Name}  & \multicolumn{1}{c|}{Definition} \\ \hline 
 logisch      & boolean      & NOT   & $y\Longleftrightarrow \neg x$ \\
 logisch      & boolean      & OR    & $y\Longleftrightarrow x_1 \vee \ldots \vee x_n$ \\
 logisch      & boolean      & AND   & $y\Longleftrightarrow x_1 \wedge \ldots \wedge x_n$ \\ \hline
 algebraisch  & geordnet     & MINUS & $y\Longleftrightarrow -x$ \\
 algebraisch  & geordnet     & INV   & $y\Longleftrightarrow x_{\text{max}}-x$ \\
 algebraisch  & geordnet     & MAX   & $y\Longleftrightarrow \text{max}(x_1,\ldots,x_n)$ \\
 algebraisch  & geordnet     & MIN   & $y\Longleftrightarrow \text{min}(x_1,\ldots,x_n)$ \\
 \hline
 \end{tabular}
 \caption{Definition einiger deterministischer Funktionen}
 \label{Deterministische Funktionen}
\end{table}

\subsection{Stochastische Verknüpfungen (ICI-Modelle)}
\label{sec:ICI models}
In der Praxis sind deterministische Beziehungen nicht besonders häufig, da das Zusammenspiel verschiedener Einflussfaktoren in der realen Welt in der Regel von Unsicherheit geprägt ist. Wird für die Elternknoten einer Beziehung in einem Bayesschen Netz aber angenommen, dass sie unabhängig in ihrem kausalen Einfluss auf einen Kindknoten sind, so lassen sich eine Reihe von Modellen für probabilistische Beziehungen formulieren, welche mit wenigen Parametern auskommen. Diese \tbf{ICI-Modelle}\footnote{Diez und Druzdzel\cite{Diez00canonicalprobabilistic} sprechen von \textit{"`independence of causal influence"'}, daher der Ausdruck \textit{"`ICI"'}.} lassen sich in zwei Klassen einteilen: Noisy und Leaky. Beide funktionieren nach demselben Prinzip, wobei im Fall eines Noisy-Modells angenommen wird, dass der betrachtete Sachverhalt vom Modell vollständig erfasst wird. Beim Leaky-Modell hingegen wird ein zusätzlicher Leak-Parameter abgeschätzt, welcher die nicht explizit modellierten Fälle abdeckt. Im Folgenden werden zunächst die beiden grundsätzlichen ICI-Klassen erklärt (Abschnitt \ref{sec:ICI models:noisy} und \ref{sec:ICI models:leaky}) und anschließend drei konkrete Noisy-ICI-Modelle abgeleitet (Abschnitt \ref{sec:ICI models:noisy:or} bis \ref{sec:ICI models:noisy:and}).

\subsubsection{Noisy-ICI-Modelle}
\label{sec:ICI models:noisy}
Noisy-ICI-Modelle lassen sich in der theoretischen Betrachtung aus deterministischen Modellen entwickeln, indem man Hilfsvariablen ${Z_1, \dots, Z_n}$ einführt, wobei $n$ die Anzahl der Elternknoten ist. Diese Hilfsvariablen dienen nur zur Erklärung des Modells, sind aber nicht Bestandteil der Modellierung. $Y$ ist eine deterministische Funktion der $Z_i$s, wärend jedes $Z_i$ probabilistisch von $X_i$ abhängt, dargestellt durch jeweils eine BWT $P(z_i|x_i)$. Diese BWTs sind die Parameter des Modells. Die bedingte Wahrscheinlichkeit $P(y|\prb x)$ berechnet sich mit  
$$P(y|\prb x) = \sum_{\prb z} P(y|\prb z) \cdot P(\prb z|\prb x),$$
wobei $P(\prb z|\prb x)$ das Produkt aller $P(z_i|x_i)$ ist:
$$P(\prb z|\prb x) = \prod_i P(z_i|x_i).$$
Für alle Noisy-ICI-Modelle gilt:
\begin{align}
\label{eq:noisy_ici}
P(y|\prb x) = \sum_{\prb z|f(\prb z)=y} \prod_i P(z_i|x_i).
\end{align}

\subsubsection{Leaky-ICI-Modelle}
\label{sec:ICI models:leaky}
Beim Noisy-ICI-Modell wird angenommen, dass alle Variablen, die Einfluss auf den Knoten $Y$ haben, im Modell explizit enthalten sind. Diese Modellierung ist aber für Probleme der realen Welt nicht immer realisierbar oder wünschenswert. In einem reduzierten Modell sind nur die Variablen des Systems explizit enthalten, für die sich die Parameter aus den zur Verfügung stehenden Daten gut ermitteln lassen oder die für den modellierten Sachverhalt besonders relevant sind. Der Einfluss implizierter Variablen $\prb V_I$ auf $Y$ kann durch den Leak-Parameter $P(z_L)$ abgeschätzt werden, wobei $Z_L$ eine virtuelle Variable ist, welche den Effekt von $\prb V_I$ zusammenfasst.
\begin{align}
P(y|\prb x) = \sum_{\prb z|f(\prb z)=y} \prod_{i|X_i \in \prb X} P(z_i|x_i) \sum_{z_L|f(\prb z,z_L)=y}P(z_L)
\end{align}

%\begin{figure}[ht!]
%\centering
%\begin{tikzpicture}[scale=1.5,auto, node distance=1cm and .5cm]
%
%\node[state]    (x1)                     {$X_1$};
%\node           (dots1) [right= of x1]    {$\cdots$};
%\node[state]    (xn)    [right= of dots1] {$X_n$};
%\node[state]    (z1)    [below= of x1]    {$Z_1$};
%\node           (dots2) [right= of z1] {$\cdots$};
%\node[state]    (zn)    [below= of xn]    {$Z_n$};
%\node[state]    (zl)    [right= of zn]    {$Z_L$};
%\node[state]    (y)     [below left= of zn] {$Y$};
%\node[state]    (air)   [below= of z1,draw=none]{};
%
%\path (x1) edge[e] (z1)
%           (z1) edge[e] (y)
%           (xn) edge[e] (zn)
%           (zn) edge[e] (y)
%           (zl) edge[e] (y);
%\draw[decorate,decoration={brace,amplitude=5pt,mirror,raise=10pt},thick]
%(x1.west) -- (z1.west) 
%node[black,midway, left, xshift=-29pt,align=center,font=\scriptsize]
%{Noisy-\\Parameter \\$P(z_i|x_i)$};
%\draw[decorate,decoration={brace,amplitude=5pt,mirror,raise=10pt},thick]
%(z1.west) -- (air.west)
%node[black,midway, left, xshift=-15pt,align=center,font=\scriptsize]
%{Deterministisches \\Modell \\(Funktion $f$)};
%\end{tikzpicture}
%\caption{Hilfsstruktur zur Ableitung eines Leaky-Modells. Die Unabhängigkeit des kausalen Einflusses wird durch das Fehlen von Verbindungen der Form $X_i\rightarrow Z_j$ und $Z_i\rightarrow Z_j$ mit $i\neq j$ verdeutlicht.}
%\end{figure}

\subsubsection{Noisy-OR}
\label{sec:ICI models:noisy:or}
Beim Noisy-OR ist $Y$ eine unscharfe OR-Verknüpfung über seinen Elternknoten $X_i$.
Interpretiert man eine Noisy-OR-Verknüpfung kausal, so ist jedes $X_i$ eine mögliche Ursache von $Y$. Die bedingten Wahrscheinlichkeiten $Z_i$ deuten an, ob $Y$ von $X_i$ erzeugt wurde. Die Bezeichnung "`noisy"' bezieht sich also auf die Möglichkeit, dass eine präsente Ursache $x_i$ keine Wirkung $y$ erzeugt. Für das hier beschriebene Modell bedeutet ein $\neg z_i$, dass $X_i$ nicht zu $Y$ geführt hat, egal, ob es mit $X_i=\neg x_i$ nicht präsent war oder ob ein Inhibitor $I_i$ verhindert hat, dass es $Y=y$ erzeugt. Mit $q_i$ wird die Wahrscheinlichkeit angegeben, dass ein solcher Inhibitor $I_i$ aktiv ist. 
\begin{Bsp}[Noisy-OR]
Sei Fieber ($F$) die Folge von Malaria ($M$), Grippe ($I$) oder Erkältung ($C$), dann bedeutet
$$q_C = P(\neg f|c,\neg i, \neg m) = 0,6,$$
dass die Erzeugung von Fieber durch Erkältung kausal unabhängig von den anderen Ursachen verhindert wurde.
Für die beiden anderen Ursachen gilt
\begin{align*}
q_I &= P(\neg f|\neg c, i, \neg m) = 0,2\text{ und} \\
q_M &= P(\neg f|\neg c, \neg i, m) = 0,1.
\end{align*}
\end{Bsp}

Die Wahrscheinlichkeit, dass $Y$ durch $X_i$ erzeugt wurde, ist 
\begin{align}
\label{eq:noisy_or_+z+x_parameter}
c_i = P(+z_i|+x_i) = 1 - q_i.
\end{align}
Wenn $X_i$ nicht auftritt, kann es $Y$ auch nicht verursachen, weshalb gilt:
\begin{align}
\label{eq:noisy_or_+z-x_parameter}
P(+z_i|\neg x_i) = 0.
\end{align}

Aus \ref{eq:noisy_or_+z+x_parameter} und \ref{eq:noisy_or_+z-x_parameter} folgt die Parameter-Tabelle für Noisy-OR:
\begin{table}[H]
\centering
\captionsetup{width=0.8\textwidth}
 \begin{tabular}{c|cc|}
  $P(z_i|x_i)$ & $+x_i$  & $\neg x_i$ \\ \hline
  $+z_i$       & $c_i$   & $0$ \\ 
  $\neg z_i$   & $1-c_i$ & $1$ \\ \hline
 \end{tabular}
\caption{Parameter in BWT-Form für Noisy-OR für die Verbindung $X_i\rightarrow Y$}
\label{Parameter-CPT Noisy-Or}
\end{table}
%Um die vollständige BWT mit Gleichung \ref{eq:noisy_ici} zu berechnen, seien zunächst $I_+$ und $I_\neg$ als Mengen der Indizes der Variablen definiert, die in einer Konfiguration binärer Elternknoten \textit{true} bzw. \textit{false} annehmen, formal ausgedrückt:
%\begin{align}
%\label{Bool-Indizes +}
%I_+(\prb v)&=\{i|V_i \mbox{ nimmt Wert }+v_i\mbox{ in }\prb v\mbox{ an}\}\\
%\label{Bool-Indizes -}
%I_\neg(\prb v)&=\{i|V_i \mbox{ nimmt Wert }\neg v_i\mbox{ in }\prb v\mbox{ an}\}.
%\end{align}
%Unter Berücksichtigung der Tatsache, dass $f_\text{OR}(\prb z)=\neg y$ nur für die Konfiguration ($\neg z_1,\ldots,\neg z_n$) gilt, ergibt sich aus Gleichung \ref{eq:noisy_ici}:
%$$P(\neg y|\prb x)=\prod_{i=1}^n P(\neg z_i|x_i)=\prod_{i\in I_+(\prb x)} P(\neg z_i|+x_i)\cdot \prod_{i\in I_\neg(\prb x)} P(\neg z_i|\neg x_i).$$
%Mit Einsetzen der Parameter aus Tabelle \ref{Parameter-CPT Noisy-Or} lautet die Berechnungsvorschrift für die vollständige bedingte Wahrscheinlichkeitsverteilung einer Noisy-OR-Verknüpfung 
%\begin{align}
%P(\neg y|\prb x) = \prod_{i\in I_+(x)} q_i = \prod_{i\in I_+(x)}(1-c_i).
%\end{align}
%Über das Gegenereignis berechnet man dann $P(+y|\prb x)= 1 - P(\neg y|\prb x)$. Die komplette Berechnung einer Tabelle für unser Fieber-Beispiel zeigt Tabelle \ref{tab:noisy-or_fever_example}.
%\begin{table}[!htbp]
%\small
%\centering
%{\renewcommand{\arraystretch}{1.2}
%\begin{tabular}{|l|l|l|l||l|}
%\hline
%Erkältung ($C$) & Grippe ($I$)   & Malaria ($M$)  & Fieber ($F$)   & $P(F|M,I,C)$               \\ \hline\hline
%\textit{false}  & \textit{false} & \textit{false} & \textit{false} & \tbf{1,0}                  \\ \hline 
%\textit{false}  & \textit{false} & \textit{false} & \textit{true}  & \tbf{0,0}                  \\ \hline
%\textit{false}  & \textit{false} & \textit{true}  & \textit{false} & \tbf{0,1}                  \\ \hline 
%\textit{false}  & \textit{false} & \textit{true}  & \textit{true}  & $\mathbf{0,9} = 1 - 0,1$   \\ \hline 
%\textit{false}  & \textit{true}  & \textit{false} & \textit{false} & \tbf{0,2}                  \\ \hline 
%\textit{false}  & \textit{true}  & \textit{false} & \textit{true}  & $\mathbf{0,8} = 1 - 0,2$   \\ \hline 
%\textit{false}  & \textit{true}  & \textit{true}  & \textit{false} & $0,02 = 0,2 \cdot 0,1$     \\ \hline 
%\textit{false}  & \textit{true}  & \textit{true}  & \textit{true}  & $0,94 = 1 - 0,02$          \\ \hline 
%\textit{true}   & \textit{false} & \textit{false} & \textit{false} & \tbf{0,6}                  \\ \hline 
%\textit{true}   & \textit{false} & \textit{false} & \textit{true}  & $\mathbf{0,4} = 1 - 0,6$   \\ \hline 
%\textit{true}   & \textit{false} & \textit{true}  & \textit{false} & $0,06 = 0,6 \cdot 0,1$     \\ \hline 
%\textit{true}   & \textit{false} & \textit{true}  & \textit{true}  & $0,94 = 1 - 0,06$          \\ \hline 
%\textit{true}   & \textit{true}  & \textit{false} & \textit{false} & $0,12 = 0,6 \cdot 0,2$     \\ \hline 
%\textit{true}   & \textit{true}  & \textit{false} & \textit{true}  & $0,88 = 1 - 0,12$          \\ \hline 
%\textit{true}   & \textit{true}  & \textit{true}  & \textit{false} & $0,012 = 0,6 \cdot 0,2 \cdot 0,1$ \\ \hline 
%\textit{true}   & \textit{true}  & \textit{true}  & \textit{true}  & $0,988 = 1 - 0,012$        \\ \hline 
%\end{tabular}}
%\caption{Noisy-OR am Beispiel von Fieberursachen: Fieber kann kausal unabhängig von Erkältung ($C$), Grippe ($I$) und Malaria ($M$) verursacht werden. Die Wahrscheinlichkeiten, dass Fieber unter einer einzelnen dieser Ursachen nicht eintritt, seien $q_C = 0,4$, $q_I = 0,2$ und $q_M = 0,1$. Mithilfe dieser Inhibitorwahrscheinlichkeiten lässt sich die komplette BWT für $P(F|M,I,C)$ berechnen. Die Werte, die in einer Parameter-BWT eines Noisy-OR auftreten, sind fett markiert.}
%\label{tab:noisy-or_fever_example}
%\end{table}

\subsubsection{Noisy-MAX}
\label{sec:ICI models:noisy:max}
Das Noisy-MAX-Modell stellt eine Verallgemeinerung des Noisy-OR für eine Variable $Y$ mit mehr als zwei Zuständen dar. $Z_i$ repräsentiert hier den Wert von $Y$, der durch $X_i$ hervorgerufen wird. Den resultierenden Wert von $Y$ liefert das größte $z_i$, es gilt also $y=f_\text{MAX}(\prb z)$. Alle  $Z_i$s müssen dieselbe Domäne haben wie $Y$. Die Noisy-MAX-Parameter für die Verbindung $X_i\rightarrow Y$ sind
\begin{align}
c_{z_i}^{x_i} = P(z_i|x_i),
\end{align}
wobei jedes $c_y^{x_i}$ als Wahrscheinlichkeit verstanden werden kann, dass $X_i$ mit dem Wert $x_i$ den Wert von $Y$ auf $y$ setzt. 
Die vollständige BWT für ein Noisy-MAX-Modell errechnet sich, indem zuerst $P(Y\leq y|\prb x)$ für alle Werte von $y$ und alle Konfigurationen $\prb x$ errechnet wird:
$$P(y\leq y|\prb x)=\sum_{\prb z|f_{\mathrm{MAX}}(\prb z)\leq y}\prod_i c_{z_i}^{x_i}=\sum_{z_1 \leq y} \cdots \sum_{z_n\leq y}\prod_i c_{z_i}^{x_i}=\prod_i\left(\sum_{z_i\leq y} c_{z_i}^{x_i}\right).$$
Man schreibt die akkumulierten Parameter
\begin{align}
\label{eq:noisy_max:accumulated_parameter}
C_y^{x_i}=\sum_{z_i\leq y} c_{z_i}^{x_i}
\end{align}
und damit
\begin{align}
\label{eq:noisy_max:accu_parameter_product}
P(Y\leq y|\prb x)=\prod_i C_y^{x_i}.
\end{align}
Die Werte der BWT können nun wie folgt errechnet werden:
\begin{align}
\label{eq:noisy_max:cpt_calculation}
P(y|\prb x) = \begin{dcases}
P(Y\leq y|\prb x) - P(Y\leq y-1|\prb x), & \mbox{ wenn }y \neq y_{\mathrm{min}} \\
P(Y\leq y|\prb x), & \mbox{ wenn }y = y_{\mathrm{min}}
\end{dcases}
\end{align}
%\begin{proof}[Beispiel]
%Man möchte den Einfluss von Migräne, Hirntumor und Clusterkopfschmerz auf die Schmerzdauer modellieren und will zwischen einer Dauer von Minuten, Stunden, Tagen, Wochen, Monaten und Jahren unterscheiden. Die Knoten dieses Modells sind also die binären Knoten $T$, $M$ und $C$ für die Schmerzursachen und der mehrwertige Knoten $S$ für die Schmerzdauer. Die Noisy-MAX-Parameter $c_{z_i}^{x_i}$ listet Tabelle \ref{tab:exmp_param_noisy_max} auf.
%Betrachte man nun eine einzelne Zeile der vollständigen BWT. Man will die Wahrscheinlichkeit für eine Schmerzdauer von Stunden bestimmen, unter der Annahme, dass der Patient nur Clusterkopfschmerz hat. Gesucht ist also $P(S = \text{h}|\neg t, \neg m, +c)$. Um den Wert zu berechnen, bestimmt man zunächst die akkumulierten Parameter (Gleichung \ref{eq:noisy_max:accumulated_parameter}):
%\begin{alignat*}{3}
%C_\text{h}^{\neg t} &= c_\text{min}^{\neg t} + c_\text{h}^{\neg t} &&= 0,2333 + 0,2333 &&= \underline{0,4666}\\
%C_\text{h}^{\neg m} &= c_\text{min}^{\neg m} + c_\text{h}^{\neg m} &&= 0,15 + 0,2 &&= \underline{0,35} \\
%C_\text{h}^{+c} &= c_\text{min}^{+c} + c_\text{h}^{+c} &&= 0,25 + 0,25 &&= \underline{0,5}. 
%\end{alignat*}
%Nun berechnet man mit Gleichung \ref{eq:noisy_max:accu_parameter_product}
%\begin{align*}
%P(S \leq \text{h}|\neg t, \neg m, +c) &= C_\text{h}^{\neg t} \cdot C_\text{h}^{\neg m} \cdot C_\text{h}^{+c}\\
%&= 0,4666 \cdot 0,25 \cdot 0,5 = \underline{0,058325}
%\end{align*}
%und
%\begin{align*}
%P(S \leq \text{min}|\neg t, \neg m, +c) &= c_\text{min}^{\neg t} \cdot c_\text{min}^{\neg m} \cdot c_\text{min}^{+c}\\
%&= 0,2333 \cdot 0,15 \cdot 0,25 = \underline{0,00874875}.
%\end{align*}
%Abschließend kann man mit Gleichung \ref{eq:noisy_max:cpt_calculation} den gesuchten Wert ausrechnen:
%\begin{align*}
%P(S=\text{h}|\neg t, \neg m, +c) &= P(S \leq \text{h}|\neg t, \neg m, +c) - P(S \leq \text{min}|\neg t, \neg m, +c) \\
%&= 0,081655 - 0,00874875 = 0.07290625 \approx \underline{\underline{0,07}}.
%\end{align*}
%\end{proof}
%\begin{table}[!htbp]
%\small
%\centering
%{\renewcommand{\arraystretch}{1.2}
%\begin{tabular}{l||l|l||l|l||l|l}
%$P(z_i|x_i)$
%&\multicolumn{2}{c|}{Hirntumor $T$}
%&\multicolumn{2}{c|}{Migräne $M$}
%&\multicolumn{2}{c}{Cluster-KS $C$} \\ \hline
%$z_i$   & $\neg t$ & $+t$   & $\neg m$ & $+m$  & $\neg c$ & $+c$  \\ \hline\hline
%Minuten (min) & 0,2333   & 0,0333 & 0,15     & 0,25  & 0,2      & 0,25  \\ \hline
%Stunden (h)   & 0,2333   & 0,0333 & 0,2      & \underline{0,25}  & 0,2      & 0,25  \\ \hline
%Tage    (d)   & 0,2333   & 0,0333 & 0,2      & 0,125 & 0,15     & 0,125 \\ \hline
%Wochen  (w)   & 0,1      & 0,1    & 0,15     & 0,125 & 0,15     & 0,125 \\ \hline
%Monate  (m)   & 0,1      & 0,4    & 0,15     & 0,125 & 0,15     & 0,125 \\ \hline
%Jahre   (y)   & 0,1      & 0,4    & 0,15     & 0,125 & 0,15     & 0,125 \\ 
%\end{tabular}}
%\caption{Parametertabellen eines Noisy-MAX für Schmerzdauer mit drei Elternknoten. Jeder Wert in einer Zelle entspricht einem Parameter $c_{z_i}^{x_i}$. So ist bspw. $c_{\text{h}}^{+m} = 0,25$. Die Werte einer Spalte müssen sich am Ende zu 1 summieren.}
%\label{tab:exmp_param_noisy_max}
%\end{table}

\subsubsection{Noisy-AND}
\label{sec:ICI models:noisy:and}
Die Elternknoten einer Noisy-AND-Verknüpfung lassen sich als Bedingungen interpretieren, die wahr sein müssen, damit $Y$ wahr wird, wobei die Unschärfe dadurch erzeugt wird, dass jede Bedingung  unterdrückt oder ersetzt werden kann. Inhibitor-Wahrscheinlichkeiten funktionieren wie beim Noisy-OR: $q_i$ ist die Wahrscheinlichkeit, dass $I_i$ aktiv ist, und wieder gilt $c_i = 1 - q_i$. Ist kein Inhibitor aktiv, ist $c_i=1$. Die Wahrscheinlichkeit, dass das $i$te Substitut $X_i$ ersetzt, wenn die Bedingung nicht erfüllt ist, wird mit $s_i$ bezeichnet, und es gilt $s_i=0$, wenn es kein Substitut für $X_i$ gibt. Allgemein gilt $c_i \cong 1$ und $s_i \cong 0$. Es ergibt sich folgende BWT eines Noisy-AND-Parameters $P(z_i|x_i)$:
\begin{table}[H]
\centering
\captionsetup{width=0.8\textwidth}
 \begin{tabular}{c|cc|}
  $P(z_i|x_i)$ & $+x_i$  & $\neg x_i$ \\ \hline
  $+z_i$       & $c_i$   & $s_i$ \\ 
  $\neg z_i$   & $1-c_i$ & $1-s_i$ \\ \hline
 \end{tabular}
\caption{Parameter in BWT-Form für Noisy-AND für die Verbindung $X_i\rightarrow Y$}
\label{Parameter-CPT Noisy-AND}
\end{table}
Die Berechnung der gesamten BWT erfolgt nach folgender Formel:
$$P(+y|\prb x) = \prod_i P(+z_i|x_i) = \prod_{i\in I_+(\prb x)}c_i\prod_{j\in I_\neg(\prb x)}s_j.$$

\section{Inferenzmechanismen}
\label{chapter:theory:sec:inference}
Dieser Abschnitt widmet sich der Fragestellung, wie mithilfe eines Bayesschen Netzes Voraussagen über Sachverhalte in der modellierten Domäne getroffen werden können. Mit der Inferenz auf einem Bayesschen Netz wird die Frage beantwortet, welche Wahrscheinlichkeitsverteilung eine Variable $X$ im Netz annimmt, unter der Voraussetzung, dass für eine Menge anderer Variablen bestimmte Werte beobachtet wurden. Diese Verteilung wird Posteriori-Verteilung genannt. 

\begin{Def}[Posteriori-Verteilung]
Die Posteriori-Verteilung wird formal ausgedrückt durch 
$$\prb P(X|\prb e),$$
wobei $\prb e$ die Menge der mit den beobachteten Werten instanziierten Beobachtungsvariablen\footnote{Beobachtungsvariablen werden auch als Evidenzvariablen bezeichnet.} ist, auch Evidenz genannt.
\end{Def}

Zunächst wird zur Veranschaulichung mit der Methode der Aufsummierung eine einfache und exakte Inferenzmethode vorgestellt (Abschnitt \ref{sec:sum_up_inference}). Es wird sich jedoch zeigen, dass der Berechnungsaufwand mit dieser Methode mit der Anzahl der Variablen exponentiell steigt. Für die Praxis sind folglich effizientere Verfahren gefragt, welche im Weiteren vorgestellt werden sollen. Der Algorithmus der Glaubenspropagation (Abschnitt \ref{sec:BP}) ist für einfach verbundene Netze effizient und exakt und es gibt mit der Inferenz in Clusterbäumen (Abschnitt \ref{sec:Junction-Tree-Inference}) und Loopy Belief Propagation (Abschnitt \ref{sec:Loopy-Belief-Propagation}) Ansätze, die ihn auch für mehrfach verbundene Netze verwendbar machen (siehe \cite[S. 529ff]{RuNo10}). Gibbs Sampling ist eine Anwendung von Monte-Carlo-Markov-Chain-Methoden (MCMC) auf die Inferenz in Bayesschen Netzen (Abschnitt \ref{sec:approx_inference}) (siehe \cite[S. 535ff]{RuNo10}). Variational Message Passing ist ein moderner Algorithmus, um auch komplexe Verteilungen effizient zu approximieren (Abschnitt \ref{chapter:theory:sec:inference:subsec:VMP}) (siehe \cite[S. 554f]{RuNo10}). Eine Übersicht über die vorgestellten Algorithmen findet sich in Tabelle \ref{Uebersicht Inferenzalgorithmen} am Ende des Kapitels. 
%Zudem wird in den einzelnen Abschnitten darauf hingewiesen, wenn ein Verfahren im Inferenzpaket Infer.NET implementiert ist, welches für den praktischen Teil dieser Arbeit verwendet und in Kapitel \ref{chapter:implementation} näher beschrieben wird.

\subsection{Inferenz durch Aufsummierung}
\label{sec:sum_up_inference}
Jede bedingte Wahrscheinlichkeit kann durch Aufsummierung der Terme aus der vollständigen gemeinsamen Verteilung berechnet werden. Für eine einzelne Abfragevariable $X$ erfolgt das mit der Gleichung
$$
\label{cond_prob_as_sum}
\prb{P}(X|\prb{e}) = \alpha\prb{P}(X,\prb{e}) = \alpha\sum_y \prb{P}(X,\prb{e},\prb{y}),$$
wobei $\alpha$ ein Normierungsfaktor ist und $\prb y$ Instanzen aller nicht beobachteten Variablen (ohne $X$) sind.

\begin{Alg}[Inferenz durch Aufsummierung]
Der Algorithmus läuft in zwei Schritten ab:
\begin{enumerate}
 \item Mit Gleichung \eqref{Verbunddichte} und Anwendung der Produktregel werden die Terme $P(x,\prb{e},\prb{y})$ als Produkte aus den bedingten Wahrscheinlichkeiten des Netzes für jede mögliche Belegung der nicht beobachteten Variablen berechnet.
 \item Anschließend werden die Einzelwahrscheinlichkeiten aufsummiert.
\end{enumerate}
\end{Alg}
 
Das Verfahren ist äquivalent zur Tiefensuche in einem Baum und hat somit eine lineare Speicherkomplexität, aber eine exponentielle Zeitkomplexität.

Wird die Berechnung in einem Ausdrucksbaum visualisiert, wird deutlich, dass viele Teilberechnungen mehrfach durchgeführt werden. Ein Zwischenspeichern der Ergebnisse dieser Berechnungen, um sie später wiederzuverwenden, senkt die benötigte Rechenzeit deutlich. Ebenso sind sämtliche Variablen, die keine Vorfahren einer Abfrage- oder Evidenzvariablen sind, für die Abfrage irrelevant und können vor der Berechnung entfernt werden. Ein Algorithmus, der dies leistet, ist die sogenannte Variableneliminierung, die in \cite{russel} beschrieben wird.

\subsection{Inferenz durch Glaubenspropagation}
\label{sec:BP}
Glaubenspropagation ist ein Inferenzverfahren, welches es ermöglicht, die Poster\-iori-Wahrscheinlichkeiten für alle Knoten des Netzes effizient zu berechnen. Die Einschränkung des Basisalgorithmus ist, dass er nur auf einfach verbundenen, also polybaumförmigen Netzen funktioniert. Zunächst soll die Kernidee des Algorithmus, das sogenannte Message Passing gezeigt werden. Danach wird beschrieben, wie dieses Prinzip auf komplexere Netze übertragen werden kann. Zum Schluss werden Ansätze diskutiert, mit denen die Einschränkungen des Basisalgorithmus teilweise aufgehoben werden.

\subsubsection{Message Passing}
\label{chapter:theory:sec:inference:subsec:BP:subsubsec:message_passing_on_chains}
Die Grundidee der Glaubenspropagation ist das iterative Aktualisieren der bedingten Wahrscheinlichkeitsverteilung eines Knotens anhand seiner Nachbarknoten. Das Prinzip soll zunächst an einem ganz einfachen Netz demonstriert werden. Dieses Netz habe eine kettenförmige Struktur, die Knoten $X_1, X_2,\dots, X_{n-1}, X_n$ seien linear aneinandergereiht.
\begin{figure}[H]
\centering
\begin{tikzpicture}[every label/.style={font=\footnotesize}]
\node[vertex] (1) at (0,0) [label=below:$X_1$]{};
\node[vertex] (2) at (1.5,0) [label=below:$X_2$]{};
\node (dots) at (3,0) {$\cdots$};
\node[vertex] (3) at (4.5,0) [label=below:$X_{n-1}$]{};
\node[vertex] (4) at (6,0) [label=below:$X_n$]{};
\path
  (1) edge[e] (2)
  (2) edge[e,shorten >=5pt] (dots)
  (dots) edge[e,shorten <=5pt] (3)
  (3) edge[e] (4);
\end{tikzpicture}
\end{figure}

\tbf{Faktorisierung der Verbunddichte} \\
%Zur Erinnerung: Die gemeinsame Verteilung dieses Netzes lässt sich als Produkt der lokalen bedingten Wahrscheinlichkeitsverteilungen seiner Variablen ausdrücken:
%$$\prb P(\prb X)=\prb P(X_1)\prb P(X_2|X_1)\prb P(X_3|X_2)\dots \prb P(X_n|X_{n-1}).$$

Die Randverteilung\footnote{Die Randverteilung, auch Marginalverteilung, wird durch die Randwahrscheinlichkeiten (Marginale) gebildet. Der Name kommt von der Randhäufigkeit, die als Summe von Häufigkeiten eines Merkmals am Rand einer Kontingenztafel steht. Randwahrscheinlichkeiten werden nach demselben Prinzip durch Aufsummierung der bedingten Wahrscheinlichkeiten einer Variable berechnet. Dieser Vorgang wird auch \tbf{Marginalisieren} genannt.} einer beliebigen Variable $X_i$ lässt sich durch Aufsummierung über alle möglichen Werte aller anderen Variablen errechnen:
$$P(X_i)=\sum_{X_1}\sum_{X_2}\cdots\sum_{X_{i-1}}\sum_{X_{i+1}}\cdots\sum_{X_n}P(\prb X).$$

\tbf{Definition der Nachrichten} \\
%Betrachtet man diese Gleichung genauer, stellt man fest, dass nur $P(X_n|X_{n-1})$ in der letzten Summe enthalten ist. Diese kann also als erstes berechnet werden und man erhält eine Funktion über $X_{n-1}$:
%$$\mu_\beta(X_{n-1})=\sum_{X_n} P(X_n|X_{n-1}).$$
Es kann nun $\mu_\beta$ iterativ auf der Knotenkette zurück bis zum gewünschten Knoten $X_i$ berechnet werdens:
\begin{align*}
\mu_\beta(X_{n-2}) &= \sum_{X_{n-1}} P(X_{n-1}|X_{n-2})\mu_\beta(X_{n-1}) \\
                   & \cdots \\
    \mu_\beta(X_i) &= \sum_{X_{i+1}} P(X_{i+1}|X_i)\mu_\beta(X_{i+1}).
\end{align*}
Ähnlich kann auch vom anderen Ende der Kette aus verfahren werden:
\begin{align*}
\mu_\alpha(X_2) &= \sum_{X_1}P(X_1)P(X_2|X_1) \\
                & \cdots \\
\mu_\alpha(X_i) &= \sum_{X_{i-1}}P(X_i|X_{i-1})\mu_\alpha(X_{i-1}).
\end{align*}
Die Randverteilung $P(X_i)$ kann nun als Produkt der von beiden Enden kommenden Beiträge berechnet werden:
$$P(X_i)=\mu_\alpha(X_i)\mu_\beta(X_i).$$

Somit kann $\mu_\alpha(X_i)$ als Nachricht aufgefasst werden, die von Knoten $X_{i-1}$ zu Knoten $X_i$ übermittelt wird, und $\mu_\beta(X_i)$ als Nachricht von Knoten $X_{i+1}$ zu Knoten $X_i$.
\begin{figure}[H]
\centering
\begin{tikzpicture}[every label/.style={font=\footnotesize}]
\node[vertex] (1) at (0,0) [label=below:$X_1$]{};
\node (dots1) at (1,0) {$\cdots$};
\node[vertex] (2) at (2,0) [label=below:$X_{i-1}$]{};
\node[vertex] (3) at (3.5,0) [label=below:$X_{i}$]{};
\node[vertex] (4) at (5,0) [label=below:$X_{i+1}$]{};
\node (dots2) at (6,0) {$\cdots$};
\node[vertex] (5) at (7,0) [label=below:$X_n$]{};
\path
  (1) edge[shorten >=-2pt] (dots1)
  (dots1) edge[shorten <=-2pt] (2)
  (2) edge (3)
  (3) edge (4)
  (4) edge[shorten >=-2pt] (dots2)
  (dots2) edge[shorten <=-2pt] (5);
\path
   (dots1.west) edge[message arrow,shorten <=10pt] node[message]{$\mu_\alpha(X_{i-1})$} (2.west)
   (2.east)     edge[message arrow]                node[message]{$\mu_\alpha(X_{i})$} (3.west)
   (3.east)     edge[message arrow,<-]             node[message]{$\mu_\beta(X_{i})$} (4.west)
   (4.east) edge[message arrow,<-,shorten >=10pt]  node[message]{$\mu_\beta(X_{i+1})$} (dots2.east);
\end{tikzpicture}
\end{figure}

Jede ausgehende Nachricht erhält man durch Multiplizieren der eingehenden Nachricht mit der lokalen bedingten Wahrscheinlichkeit und Aufsummieren über alle möglichen Werte des sendenden Knotens.

\tbf{Vollständiges Message Passing} \\
Um die Randwahrscheinlichkeiten aller Knoten $X_i$ der Kette zu berechnen, verfährt man nach folgendem Schema:
\begin{enumerate}
\item Senden der Nachrichten $\mu_\alpha$, mit $\mu_\alpha(X_1)$ beginnend bis $\mu_\alpha(X_n)$.
\item Zurücksenden der Nachrichten $\mu_\beta$, mit $\mu_\beta(X_n)$ beginnend bis $\mu_\beta(X_1)$.
\end{enumerate}
%Speichert man die Nachrichten für jeden Knoten, so erhält man alle Randwahrscheinlichkeiten durch das Multiplizieren der beiden Nachrichten jedes Knotens. Um die Randverteilungen für das gesamte Netz zu erhalten, wird somit nur die doppelte Anzahl an Nachrichtenübermittlungen benötigt wie für das Ermitteln einer einzelnen Randverteilung.

\tbf{Berücksichtigung von Evidenz} \\
Möchte man nun die Posteriori-Wahr\-schein\-lich\-keit unter gegebenen Beobachtungen $\prb e$ berechnen, so verwendet man beim Berechnen der Nachrichten des beobachteten Knotens einfach den beobachteten Wert, statt über alle möglichen Werte des Knotens aufzusummieren. Anschließend muss normalisiert werden:
\begin{align}
\prb P(X_i|\prb e)=\frac{\prb P(X_i,\prb e)}{\sum_{X_i}P(X_i,\prb e)}.
\end{align}

Im Abschnitt \ref{sec:message_passing_on_factor_graphs} wird das eben beschriebene Message-Passing-Schema auf beliebige Polybaumnetze verallgemeinert. Dafür wird jedoch eine geeignetere graphische Struktur benötigt, die im nächsten Abschnitt eingeführt wird.

\subsubsection{Faktorgraphen}
Wie schon im letzten Abschnitt gezeigt, macht sich Glaubenspropagation die Faktorisierung von Bayesschen Netzen für eine iterative Berechnung zunutze. Daher lässt sie sich auf einer graphischen Struktur, die diese Faktorisierung besonders hervorhebt, leichter implementieren und erklären.  

\begin{Def}[Faktorgraph]
Ein Faktorgraph ist ein bibartiter Graph\footnote{Bibartite Graphen beschreiben die Beziehungen zwischen den Elementen zweier Mengen.} mit folgenden Eigenschaften:
\begin{itemize}
 \item Er besteht aus zwei verschiedenen Knotentypen, Variablen und Faktoren, sowie ungerichteten Kanten zwischen jeweils einer Variable und einem Faktor.\footnote{Wie beim Bayesschen Netz die Begriffe \textit{Knoten} und \textit{Variablen} werden beim Faktorgraphen die Begriffe \textit{Faktor} und \textit{Faktorknoten} synonym verwendet, wobei der erste Begriff eher im statistischen und der zweite eher im graphisch-strukturellen Kontext verwendet wird. Für die Knoten der Variablenmenge wird der Begriff \textit{Variable} oder \textit{Variablenknoten} verwendet.}
 \item Ein Knoten der Variablenmenge repräsentiert eine Zufallsvariable $X_i$ und wird durch einen Kreis dargestellt.
 \item Ein Knoten der Faktormenge repräsentiert einen Faktor $f_j$, dargestellt durch ein Quadrat. Dieser beschreibt eine Wahrscheinlichkeitsverteilung über die angrenzenden Zufallsvariablen. Dies kann eine bedingte Wahrscheinlichkeitsverteilung, aber auch das Produkt von Wahrscheinlichkeitsverteilungen bis hin zu einer Verbundwahrscheinlichkeit sein (Abbildung \ref{fig:factor_graph} b) und c)).
\end{itemize}
\end{Def}
%\vspace{1cm}

Das Bayessche Netz in Abbildung \ref{fig:factor_graph} a) kann in äquivalente Faktorgraphen umgewandelt werden. Die A-Priori-Wahrscheinlichkeiten der Knoten $X_1$ und $X_2$ können b) direkt in einem Faktor zusammengefasst oder c) in separaten Faktoren modelliert werden.

\begin{figure}[!tbp]
%\begin{figure}[!ht]
\centering
\scalebox{0.7}{\begin{tikzpicture}[every label/.style={font=\small}]
\tikzstyle{vertex}=[circle, draw, font=\small, inner sep=0pt, minimum size=25pt]
\tikzstyle{phantom}=[vertex,draw=none]
\tikzstyle{factor}=[draw, fill, inner sep=0pt, minimum size=15pt]
\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]

\node (A) at (0,0){
\begin{tikzpicture}
\node[vertex] (g1_x1) at (0,2.85) [label=above left : $X_1$]{};
\node[vertex] (g1_x2) at (3,2.85) [label=above right: $X_2$]{};
\node[vertex] (g1_x3) at (1.5,0) [label=below right: $X_3$]{};
\path
    (g1_x1) edge[e] (g1_x3)
    (g1_x2) edge[e] (g1_x3);
\draw[description] (g1_x3) node{$P(X_3|X_2,X_1)P(X_1)P(X_2)$};
\end{tikzpicture}};
\draw[decorate,font=\large] (A.north west) node[above right=-4pt]{a)};

\node[below right=0 and -1.5 of A.north east] (B){
\begin{tikzpicture}
\node[vertex] (g2_x1) at (0,3)   [label=above left : $X_1$]{};
\node[vertex] (g2_x2) at (3,3)   [label=above right: $X_2$]{};
\node[phantom] (g2_v1) at (1.5,3) {}; % virtual node for positioning
\node[factor, below=0.5 of g2_v1] (g2_f)  [label=above      : $f$]{};
\node[vertex, below=0.9 of g2_f]  (g2_x3) [label=below right: $X_3$]{};
\path
    (g2_x1) edge (g2_f)
    (g2_x2) edge (g2_f)
    (g2_x3) edge (g2_f);
\draw[description] (g2_x3) node{$f(X_1,X_2,X_3)=P(X_3|X_2,X_1)P(X_1)P(X_2)$};
\end{tikzpicture}};
\draw[decorate,font=\large] (B.north west) node[above right=-4pt and 30pt]{b)};

\node[below right=0 and -1.5 of B.north east] (C){
\begin{tikzpicture}
\node[vertex] (g3_x1) at (0,3)            [label=above left : $X_1$]{};
\node[vertex] (g3_x2) at (3,3)            [label=above right: $X_2$]{};
\node[phantom] (g3_v1) at (1.5,3) {}; % virtual node for positioning
\node[factor, below=0.5 of g3_x1] (g3_fa) [label=left       : $f_a$]{};
\node[factor, below=0.5 of g3_x2] (g3_fb) [label=right      : $f_b$]{};
\node[factor, below=0.5 of g3_v1] (g3_fc) [label=above      : $f_c$]{};
\node[vertex,below=0.9 of g3_fc]  (g3_x3) [label=below right: $X_3$]{};
\path
    (g3_x1) edge (g3_fa)
    (g3_x2) edge (g3_fb)
    (g3_x1) edge (g3_fc)
    (g3_x2) edge (g3_fc)
    (g3_x3) edge (g3_fc);
\draw[description] (g3_x3) node{$f_a(X_1)=P(X_1)$\\
$f_b(X_2)=P(X_2)$\\
$f_c(X_1,X_2,X_3)=P(X_3|X_2,X_1)$};
\end{tikzpicture}};
\draw[decorate,font=\large] (C.north west) node[above right=-4pt and 10pt]{c)};
\end{tikzpicture}}
\caption{Bayessches Netz und äquivalente Faktorgraphen}
\label{fig:factor_graph}
\end{figure}

Jedes Bayessche Netz lässt sich durch einen Faktorgraphen darstellen.\footnote{Der Beweis dafür basiert auf dem sogenannten \tbf{Hammersley-Clifford-Theorem}.\cite{DBLP:journals/corr/abs-1207-1366}} Die Vorgehensweise zur Bildung eines solchen äquivalenten Faktorgraphen ist wie folgt.

\begin{Alg}[Bildung eines Faktorgraphen]
\begin{enumerate}
 \item Für jeden Knoten des Bayesschen Netzes wird ein Variablenknoten erzeugt.
 \item Für jeden Kindknoten des Bayesschen Netzes wird ein Faktorknoten mit der bedingten Wahrscheinlichkeitsverteilung des Kindknotens erzeugt. Anschließend wird der Faktorknoten mittels ungerichteter Kanten mit den äquivalenten Variablenknoten der Elternknoten des Kindknotens und dem Kindknoten selbst verbunden.
 \item Für jeden Wurzelknoten wird ein Faktor mit der A-Priori-Wahr\-schein\-lich\-keit des jeweiligen Wurzelknotens erzeugt und verbindet ihn durch eine ungerichtete Kante mit der äquivalenten Variable des Wurzelknotens (Abbildung \ref{fig:factor_graph} c)).\\
 Alternativ: Es wird die A-Priori-Wahrscheinlichkeit jedem Faktorknoten hinzugefügt, der an den zum Wurzelknoten äquivalenten Variablenknoten angrenzt, indem sie mit diesem Faktor multipliziert wird (Abbildung \ref{fig:factor_graph} b)).
\end{enumerate}
\end{Alg}

\subsubsection{Summe-Produkt-Algorithmus auf Faktorgraphen}
\label{sec:message_passing_on_factor_graphs}
Der Summe-Produkt-Algorithmus ist ein effizientes Verfahren für exakte Inferenz auf baumartig strukturierten Graphen. Er ist eine Verallgemeinerung des zuvor auf dem kettenartigen Netz gezeigten Message-Passing-Algorithmus.

Gesucht ist die Randverteilung von $X$:
$$\prb P(X)=\sum_{\prb X \backslash X}\prb P(\prb X).$$
Verallgemeinert man das Message-Passing-Schema für kettenförmige Graphen, so berechnet man die Randwahrscheinlichkeit als das Produkt der Nachrichten, die von allen benachbarten Faktoren $f_i \in \mathcal N(X)$ kommen (Abbildung \ref{General Message Passing}):
$$P(X)=\prod_{f_i\in \mathcal N(X)}\mu_{f_i\rightarrow x}(X).$$

\begin{figure}[!tbp]
\centering
\scalebox{0.8}{
\begin{tikzpicture}[every label/.style={font=\small}]
\tikzstyle{vertex}=[circle, draw, font=\scriptsize, inner sep=0pt, minimum size=25pt]
\tikzstyle{factor}=[draw, fill, inner sep=0pt, minimum size=15pt]
\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]
\tikzstyle{phantom}=[vertex,draw=none]
\tikzstyle{dots}=[loosely dotted,shorten <=3pt, shorten >=3pt]
\tikzstyle{message}=[above,font=\footnotesize,sloped, inner sep=13pt]
\tikzstyle{message arrow}=[->,>=stealth,
     shorten >=10pt, shorten <=10pt, 
     decoration={sl,raise=8pt},decorate]

\node[vertex] (x1) at (0,0){};
\node[factor,draw=none,fill=none,below=0.1 of x1] (pf1) {};
\node[vertex,  below=0.7 of x1] (x2){};
\node[phantom, below=1.5 of x1] (px) {};
\node[factor,  right=1.2 of pf1] (f1)[label={above,align=center:$\hspace{70pt}\mathcal N(X)=\{f_1,\dots,f_n\}$\\$f_1$}]{};
\node[vertex,  right=4 of px] (x) [label={below:$X$}]{};
\node[vertex,  below=2 of x1] (x3){};
\node[phantom, below=2.7 of x1] (pf2) {};
\node[factor,  below=2.3 of f1] (f2)[label={below:$f_n$}]{};
\node[vertex,  below=3.7 of x1] (x4){};

\path
    (x1) edge[dots] (x2)
    (x2) edge[dots] (x3)
    (x3) edge[dots] (x4)
    (f1) edge[dots] (f2)
    (x1) edge (f1)
    (x2) edge (f1)
    (x3) edge (f2)
    (x4) edge (f2)
    (f1) edge (x)
    (f2) edge (x)
    (f1) edge[message arrow] node[message]{$\mu_{f_1\rightarrow X}(X)$} (x)
    (f2) edge[message arrow] node[message]{$\mu_{f_n\rightarrow X}(X)$} (x);
\end{tikzpicture}}
\caption{Die Randverteilung $P(X)$ eines Knotens $X$ berechnet sich durch Multiplikation der eingehenden Knotennachrichten $\mu_{f_1\rightarrow X}(X),\ldots \mu_{f_1\rightarrow X}(X)$ von allen benachbarten Faktoren $f_1,\ldots,f_n$.}
\label{General Message Passing}
\end{figure}
In einem Faktorgraphen werden zwei Typen von Nachrichten unterschieden: die Faktornachricht von einem Faktor $f_s$ zu einem Knoten $X$ und die Knotennachricht von einem Knoten $X_j$ an einen Faktor $f_s$.

\tbf{Faktornachricht} \\
Eine Faktornachricht an Knoten $X$ ist das Produkt der in den Faktorknoten $f_s$ eingehenden Nachrichten von allen benachbarten Variablenknoten außer von $X$, multipliziert mit dem Faktor, welcher über allen möglichen Werten aller im Faktor vorkommenden Variablen außer $X$ aufsummiert wird:
\begin{align}
\label{eq:factor_message}
\mu_{f_s\rightarrow X}(X)=
    \sum_{X_1}\cdots\sum_{X_m}f_s(X,X_1,\dots,X_m)
    \prod_{X_j\in \mathcal N(f_s)\backslash X} \mu_{X_j\rightarrow f_s}(X_j).
\end{align}
    
%\begin{figure}[!htbp]
% \centering
%\scalebox{0.8}{
%\begin{tikzpicture}[every label/.style={font=\small}]
%\tikzstyle{vertex}=[circle, draw, font=\scriptsize, inner sep=0pt, minimum size=25pt]
%\tikzstyle{factor}=[draw, fill, inner sep=0pt, minimum size=15pt]
%\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]
%\tikzstyle{phantom}=[factor,draw=none,fill=none]
%\tikzstyle{dots}=[loosely dotted,shorten <=3pt, shorten >=3pt]
%\tikzstyle{message}=[above,font=\footnotesize,sloped, inner sep=13pt]
%\tikzstyle{message arrow}=[->,>=stealth,
%     shorten >=10pt, shorten <=10pt, 
%     decoration={sl,raise=8pt},decorate]
%
%\node[vertex] at (0,0) (x1)[label={above,align=center:$\mathcal N(f_s)\backslash X$\\$X_1$}]{};
%\node[phantom, below=0.3 of x1] (pfs) {};
%\node[factor,  right=2 of pfs] (fs) [label={below:$f_s$}]{};
%\node[vertex,  below=1.5 of x1] (xl)[label={below:$X_m$}]{};
%\node[vertex,  right=2 of fs] (x)[label={below:$X$}]{};
%
%\path
%    (x1) edge[dots] (xl)
%    (x1) edge (fs)
%    (xl) edge (fs)
%    (fs)  edge (x)
%    (x1) edge[message arrow] node[message]{$\mu_{X_1\rightarrow f_s}(X_1)$} (fs)
%    (fs) edge[message arrow] node[message]{$\mu_{f_s\rightarrow X}(X)$} (x);
%
%\end{tikzpicture}}
%\caption{Die Faktornachricht $\mu_{f_s\rightarrow X}(X)$ berechnet sich durch Multiplikation der eingehenden Knotennachrichten $\mu_{X_1\rightarrow f_s}(X),\ldots,\mu_{X_m\rightarrow f_s}(X_m)$ aller benachbarten Variablenknoten $X_1,\ldots,X_m$ (außer Knoten $X$) mit dem Faktor $f_s$, aufsummiert über alle Werte der Variablen $X_1,\ldots,X_m$.}
%\end{figure}

\tbf{Knotennachricht} \\
Eine Knotennachricht an einen Faktor $f_s$ ist das Produkt der in den Knoten $X$ eingehenden Faktornachrichten von allen anderen Faktoren, außer $f_s$:
\begin{align}
\label{eq:variable_message}
\mu_{X\rightarrow f_s}(X)=\prod_{f_i\in\mathcal N(X)\backslash f_s} \mu_{f_i\rightarrow X}(X).
\end{align}
%\begin{figure}[!htbp]
% \centering
%\scalebox{0.8}{
%\begin{tikzpicture}[every label/.style={font=\small}]
%\tikzstyle{vertex}=[circle, draw, font=\scriptsize, inner sep=0pt, minimum size=25pt]
%\tikzstyle{factor}=[draw, fill, inner sep=0pt, minimum size=15pt]
%\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]
%\tikzstyle{phantom}=[vertex,draw=none]
%\tikzstyle{dots}=[loosely dotted,shorten <=3pt, shorten >=3pt]
%\tikzstyle{message}=[above,font=\footnotesize,sloped, inner sep=13pt]
%\tikzstyle{message arrow}=[->,>=stealth,
%     shorten >=10pt, shorten <=10pt, 
%     decoration={sl,raise=8pt},decorate]
%
%\node[factor] at (0,0) (f1)[label={above,align=center:$\mathcal N(X)\backslash f_s$\\$f_1$}]{};
%\node[phantom, below=0.75 of f1] (px) {};
%\node[vertex,  right=2 of px] (x) [label={below:$X$}]{};
%\node[factor,  below=2.3 of f1] (f2)[label={below:$f_l$}]{};
%\node[factor,  right=2 of x] [label={below:$f_s$}](fs){};
%
%\path
%    (f1) edge[dots] (f2)
%    (f1) edge (x)
%    (f2) edge (x)
%    (x)  edge (fs)
%    (x) edge[message arrow] node[message]{$\mu_{X\rightarrow f_s}(X)$} (fs)
%    (f1) edge[message arrow] node[message]{$\mu_{f_1\rightarrow X}(X)$} (x);
%
%\end{tikzpicture}}
%\caption{Die Knotennachricht $\mu_{X\rightarrow f_s}(X)$ berechnet sich durch Multiplikation der eingehenden Faktornachrichten $\mu_{f_1\rightarrow X}(X),\ldots,\mu_{f_l\rightarrow X}(X)$ aller beachbarten Faktoren $f_1,\ldots,f_l$ außer dem Faktor $f_s$.}
%\label{fig:node_message}
%\end{figure}

\tbf{Initialisierung} \\
Bevor der eigentliche Message-Passing-Algorithmus startet, müssen die Nachrichten der Blätter des Graphen initialisiert werden. Ein Blatt kann sowohl ein Faktor, als auch eine Variable sein. 
%\begin{figure}[H]
% \centering
% \scalebox{0.8}{
%\begin{tikzpicture}[every label/.style={font=\small}]
%\tikzstyle{vertex}=[circle, draw, font=\scriptsize, inner sep=0pt, minimum size=25pt]
%\tikzstyle{factor}=[draw, fill, inner sep=0pt, minimum size=15pt]
%\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]
%\tikzstyle{phantom}=[vertex,draw=none]
%\tikzstyle{dots}=[loosely dotted,shorten <=3pt, shorten >=3pt]
%\tikzstyle{message}=[above, inner sep=20pt,xshift=5pt]
%\tikzstyle{message arrow}=[->,>=stealth,
%     shorten >=10pt, shorten <=10pt, 
%     decoration={sl,raise=8pt},decorate]
%
%\node[factor] at (0,0)       (f) [label={below:$f$}]{};
%\node[vertex, right=2 of f] (x) [label={below:$X$}]{};
%
%\path
%    (f) edge (x)
%    (f) edge[message arrow] node[message]{$\mu_{f\rightarrow X}(X)=f(X)$} (x);
%\end{tikzpicture}}
%\caption{Ist das Blatt ein Faktor, so wird die Nachricht mit dem Faktor selbst initialisiert.}
%\label{Init Factor}
%\end{figure}
%
%\begin{figure}[H]
% \centering
% \scalebox{0.8}{
%\begin{tikzpicture}[every label/.style={font=\small}]
%\tikzstyle{vertex}=[circle, draw, font=\scriptsize, inner sep=0pt, minimum size=25pt]
%\tikzstyle{factor}=[draw, fill, inner sep=0pt, minimum size=15pt]
%\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]
%\tikzstyle{phantom}=[vertex,draw=none]
%\tikzstyle{dots}=[loosely dotted,shorten <=3pt, shorten >=3pt]
%\tikzstyle{message}=[above, inner sep=20pt]
%\tikzstyle{message arrow}=[->,>=stealth,
%     shorten >=10pt, shorten <=10pt, 
%     decoration={sl,raise=8pt},decorate]
%
%\node[vertex] at (0,0)      (x) [label={below:$X$}]{};
%\node[factor, right=2 of x] (f) [label={below:$f$}]{};
%
%\path
%    (x) edge (f)
%    (x) edge[message arrow] node[message]{$\mu_{X\rightarrow f}(X)=1$} (f);
%\end{tikzpicture}}
%\caption{Ist das Blatt eine Variable, so wird die Nachricht mit dem Wert $1$ initialisiert.}
%\label{Init Variable}
%\end{figure}

\tbf{Vollständiges Message Passing} \\
Um die Randwahrscheinlichkeiten für alle Knoten des Graphen zu berechnen, müssen Nachrichten über alle Kanten des Graphen jeweils in beide Richtungen geschickt werden. Ähnlich wie beim Message Passing auf einer Knotenkette (Abschnitt \ref{chapter:theory:sec:inference:subsec:BP:subsubsec:message_passing_on_chains}) läuft der Algorithmus in zwei Phasen ab. Nach Initialisierung der Blätter wird zunächst ein beliebiger Knoten des Graphen als Wurzelknoten gewählt. 
\begin{enumerate}
 \item In Phase 1 werden, von den Blattknoten ausgehend, die Nachrichten in Richtung des Wurzelknoten geschickt.
 % (Abbildung \ref{Faktor-Graph MP Example Phase 1}).
 \item In Phase 2 werden, vom Wurzelknoten ausgehend, die Nachrichten zurück in die Blattknoten geschickt.
 % (Abbildung \ref{Faktor-Graph MP Example Phase 2}).
\end{enumerate}
%\begin{figure}[!bp]
%\centering
%\scalebox{0.8}{
%\begin{tikzpicture}[every label/.style={font=\small}]
%\tikzstyle{vertex}=[circle, draw, font=\scriptsize, inner sep=0pt, minimum size=25pt]
%\tikzstyle{factor}=[draw, fill, inner sep=0pt, minimum size=15pt]
%\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]
%\tikzstyle{phantom}=[vertex,draw=none]
%\tikzstyle{dots}=[loosely dotted,shorten <=3pt, shorten >=3pt]
%\tikzstyle{message}=[above, inner sep=20pt,font=\footnotesize]
%\tikzstyle{message arrow}=[->,>=stealth,
%     shorten >=10pt, shorten <=10pt, 
%     decoration={sl,raise=8pt},decorate,sloped]
%
%\node[vertex] at (0,0)         (x1) [label={below:$X_1$}]{};
%\node[factor, right=1.5 of x1] (fa) [label={below:$f_a$}]{};
%\node[vertex, right=1.5 of fa] (x2) [label={below right:$X_2$}]{};
%\node[factor, right=1.5 of x2] (fb) [label={below:$f_b$}]{};
%\node[vertex, right=1.5 of fb] (x3) [label={below:$X_3$}]{
%\begin{tikzpicture}
%\node[vertex, fill, minimum size=10pt] (xf) {};
%\end{tikzpicture}
%};
%\node[factor, below=1.5 of x2] (fc) [label={right:$f_c$}]{};
%\node[vertex, below=1.5 of fc] (x4) [label={below:$X_4$}]{};
%
%\path
%  (x1) edge (fa)
%  (x1) edge[message arrow] node[message]{$\mu_{X_1\rightarrow f_a}(X_1)$} (fa)
%  (fa) edge (x2)
%  (fa) edge[message arrow] node[message]{$\mu_{f_a\rightarrow X_2}(X_2)$} (x2)
%  (x2) edge (fb)
%  (x2) edge[message arrow] node[message]{$\mu_{X_2\rightarrow f_b}(X_2)$} (fb)
%  (fb) edge (x3)
%  (fb) edge[message arrow] node[message]{$\mu_{f_b\rightarrow X_3}(X_3)$} (x3)
%  (x2) edge (fc)
%  (fc) edge[message arrow] node[message]{$\mu_{f_c\rightarrow X_2}(X_2)$} (x2)
%  (fc) edge (x4)
%  (x4) edge[message arrow] node[message]{$\mu_{X_4\rightarrow f_a}(X_4)$} (fc);
%\end{tikzpicture}}
%\caption{Beispiel Message Passing auf einem Faktorgraphen, Phase 1:\\Senden der Nachrichten von den Blättern in Richtung des Wurzelknotens $X_3$. Das Verschicken der Nachrichten entlang der Äste $X_1 \rightarrow X_2$ und $X_4 \rightarrow X_2$ kann parallel erfolgen.}
%\label{Faktor-Graph MP Example Phase 1}
%\end{figure}

Werden für jeden Variablenknoten die Nachrichten zwischengespeichert, so kann anschließend für jede Variable die Randwahrscheinlichkeit durch Multiplikation dieser Nachrichten bestimmt werden. Für das Berechnen aller Randwahrscheinlichkeiten wird auch hier wieder nur die doppelte Anzahl an Nachrichtenübermittlungen benötigt wie für das Berechnen der Randwahrscheinlichkeit für eine einzelne Variable.

%\begin{figure}[!tbp]
%\centering
%\scalebox{0.8}{
%\begin{tikzpicture}[every label/.style={font=\small}]
%\tikzstyle{vertex}=[circle, draw, font=\scriptsize, inner sep=0pt, minimum size=25pt]
%\tikzstyle{factor}=[draw, fill, inner sep=0pt, minimum size=15pt]
%\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]
%\tikzstyle{phantom}=[vertex,draw=none]
%\tikzstyle{dots}=[loosely dotted,shorten <=3pt, shorten >=3pt]
%\tikzstyle{message}=[above, inner sep=20pt,font=\footnotesize]
%\tikzstyle{message arrow}=[->,>=stealth,
%     shorten >=10pt, shorten <=10pt, 
%     decoration={sl,raise=8pt},decorate,sloped]
%
%\node[vertex] at (0,0)         (x1) [label={below:$X_1$}]{};
%\node[factor, right=1.5 of x1] (fa) [label={below:$f_a$}]{};
%\node[vertex, right=1.5 of fa] (x2) [label={below right:$X_2$}]{};
%\node[factor, right=1.5 of x2] (fb) [label={below:$f_b$}]{};
%\node[vertex, right=1.5 of fb] (x3) [label={below:$X_3$}]{
%\begin{tikzpicture}
%\node[vertex, fill, minimum size=10pt] (xf) {};
%\end{tikzpicture}
%};
%\node[factor, below=1.5 of x2] (fc) [label={right:$f_c$}]{};
%\node[vertex, below=1.5 of fc] (x4) [label={below:$X_4$}]{};
%
%\path
%  (x1) edge (fa)
%  (x1) edge[message arrow,<-] node[message]{$\mu_{f_a\rightarrow X_1}(X_1)$} (fa)
%  (fa) edge (x2)
%  (fa) edge[message arrow,<-] node[message]{$\mu_{X_2\rightarrow f_a}(X_2)$} (x2)
%  (x2) edge (fb)
%  (x2) edge[message arrow,<-] node[message]{$\mu_{f_b\rightarrow X_2}(X_2)$} (fb)
%  (fb) edge (x3)
%  (fb) edge[message arrow,<-] node[message]{$\mu_{X_3\rightarrow f_b}(X_3)$} (x3)
%  (x2) edge (fc)
%  (fc) edge[message arrow,<-] node[message]{$\mu_{X_2\rightarrow f_c}(X_2)$} (x2)
%  (fc) edge (x4)
%  (x4) edge[message arrow,<-] node[message]{$\mu_{f_a\rightarrow X_4}(X_4)$} (fc);
%\end{tikzpicture}}
%\caption{Beispiel Message Passing auf einem Faktorgraphen, Phase 2:\\Senden der Nachrichten vom Wurzelknoten $X_3$ zu den Blättern $X_1$ und $X_4$. Das Verschicken der Nachrichten entlang der Äste $X_2 \rightarrow X_1$ und $X_2 \rightarrow X_4$ kann parallel erfolgen.}
%\label{Faktor-Graph MP Example Phase 2}
%\end{figure}

%\enlargethispage{2\baselineskip}
%\begin{proof}[Beispiel] Zur Veranschaulichung sei ein Graph mit vier Variablen $X_1,X_2,X_3,X_4$ und drei Faktoren $f_a,f_b,f_c$ gegeben und die Verbunddichte als Produkt der Faktoren sei
%$$P(\prb X)=f_a(X_1,X_2)f_b(X_2,X_3)f_c(X_2,X_4).$$
%\begin{enumerate}
% \item Wähle $X_3$ als Wurzelknoten.
% \item Initialisiere die Nachrichten der Blätter $X_1$ und $X_4$ mit
% \begin{align*}
%   \mu_{X_1\rightarrow f_a}(X_1)&=1\\
%   \mu_{X_4\rightarrow f_c}(X_4)&=1.
% \end{align*}
% \item Phase 1: Sende Nachrichten von den Blättern zum Wurzelknoten (Abbildung \ref{Faktor-Graph MP Example Phase 1}):
% \begin{enumerate}
%   \item Sende Nachricht $\mu_{X_1\rightarrow f_a}(X_1)$ an $f_a$ und $\mu_{X_4\rightarrow f_c}(X_4)$ an $f_c$.
%   \item Sende Nachrichten von den Faktorknoten $f_a$ und $f_b$ zu Knoten $X_2$ mit
%   \begin{align*}
%     \mu_{f_a\rightarrow X_2}(X_2)=\sum_{X_1}f_a(X1,X2) \\
%     \mu_{f_c\rightarrow X_2}(X_2)=\sum_{X_4}f_c(X2,X4).
%   \end{align*}
%   \item Sende Nachricht von Knoten $X_2$ zu Faktorknoten $f_b$ mit
%   $$\mu_{X_2\rightarrow f_b}(X_2)=\mu_{f_a\rightarrow X_2}(X_2)\mu_{f_c\rightarrow X_2}(X_2).$$
%   \item Sende Nachricht von $f_b$ zu Knoten $X_3$ mit
%   $$\mu_{f_b\rightarrow X_3}(X_3)=\sum_{X_2}f_b(X_2,X_3)\mu_{X_2\rightarrow f_b}(X_2).$$
% \end{enumerate}
% \item Phase 2: Sende Nachrichten vom Wurzelknoten zu den Blättern (Abbildung \ref{Faktor-Graph MP Example Phase 2}):
%   \begin{enumerate}
%     \item Sende Nachricht von Faktorknoten $f_b$ zu $X_3$ mit
%       $$\mu_{f_b\rightarrow X_3}(X_3)=\sum_{X_2}f_b(X_2,X_3)\mu_{X_2\rightarrow f_b}(X_2).$$
%     \item Sende Nachricht von Wurzelknoten $X_3$ mit
%       $$\mu_{X_3\rightarrow f_b}(X_3)=1.$$
%     \item Sende Nachricht von Faktor $f_b$ zu Knoten $X_2$ mit
%       $$\mu_{f_b\rightarrow X_2}(X_2)=\sum_{X_3}f_b(X_2,X_3).$$
%     \item Sende Nachrichten von $X_2$ zu Faktorknoten $f_a$ und $f_b$ mit
%     \begin{align*}
%       \mu_{X_2\rightarrow f_a}(X_2)=\mu_{f_b\rightarrow X_2}(X_2)\mu_{f_c\rightarrow X_2}(X_2) \\
%       \mu_{X_2\rightarrow f_c}(X_2)=\mu_{f_b\rightarrow X_2}(X_2)\mu_{f_a\rightarrow X_2}(X_2).
%     \end{align*}
%     \item Sende Nachrichten von Faktoren $f_a$ und $f_c$ zu Knoten $X_1$ und $X_4$:
%     \begin{align*}
%       \mu_{f_a\rightarrow X_1}(X_1)=\sum_{X_2}f_a(X_1,X_2)\mu_{X_2\rightarrow f_a}(X_2) \\
%       \mu_{f_a\rightarrow X_4}(X_4)=\sum_{X_2}f_c(X_2,X_4)\mu_{X_2\rightarrow f_c}(X_2).
%     \end{align*}
%   \end{enumerate}
%\end{enumerate}
%
%Nun soll exemplarisch für den Knoten $X_2$ aus den empfangenen Nachrichten die Marginalwahrscheinlichkeit berechnet werden:
%\begin{align*}
%P(X_2)&=\mu_{f_a\rightarrow X_2}(X_2)\mu_{f_b\rightarrow X_2}(X_2)\mu_{f_c\rightarrow X_2}(X_2) \\
%&=\left[\sum_{X_1}f_a(X_1,X_2)\right]\left[\sum_{X_3}f_b(X_2,X_3)\right]\left[\sum_{X_4}f_c(X_2,X_4)\right] \\
%&=\sum_{X_1}\sum_{X_3}\sum_{X_4}f_a(X_1,X_2)f_b(X_2,X_3)f_c(X_2,X_4)\\
%&=\sum_{X_1}\sum_{X_3}\sum_{X_4}P(\prb X).
%\end{align*}
%\end{proof}

\tbf{Berücksichtigung von Evidenz} \\
Möchte man Posteriori-Wahrscheinlichkeiten unter gegebenen Beobachtungen berechnen, verwendet man die beobachteten Werte der Evidenzvariablen\footnote{Variablenknoten des Graphen, für die ein bestimmter Wert beobachtet wird.}, um Faktornachrichten zu berechnen, statt über alle ihre Werte aufzusummieren (analog zu Abschnitt \ref{chapter:theory:sec:inference:subsec:BP:subsubsec:message_passing_on_chains}). Gleichung \ref{eq:factor_message} ändert sich unter Beobachtung des Knotens $X_i$ mit dem Wert $e_i$ wie folgt: 
\begin{align}
\mu_{f_s\rightarrow X}(X)=
    \sum_{X_1}\cdots\sum_{X_{i-1}}\sum_{X_{i+1}}\cdots\sum_{X_m}f_s(X,X_1,\dots,e_i,\dots,X_m)
    \prod_{X_j\in \mathcal N(f_s)\backslash X} \mu_{X_j\rightarrow f_s}(X_j).
\end{align}

Die Berechnung der Posteriori-Wahr\-schein\-lich\-keiten für die einzelnen Knoten $X_i$ unter gegebener Evidenz $\prb e$ erfolgt, wie die Berechnung der Randwahrscheinlichkeiten ohne Evidenz, durch Multiplikation der eingehenden Faktornachrichten, wobei mit dem Faktor $\frac{1}{\sum_{X}P(X,\prb e)}$ normalisiert werden muss.
\begin{align}
\prb P(X|\prb e) = \frac{\prod_i \mu_{f_i\rightarrow X}(X)}{\sum_X \prod_i \mu_{f_i\rightarrow X}(X)}.
\end{align}

\subsubsection{Exakte Inferenz auf verbundenen Netzen mit Junction Trees}
\label{sec:Junction-Tree-Inference}
Ein verbundenes Bayessches Netz liefert einen Faktorgraphen mit Schleifen. Auf einem solchen Graphen ist mit dem Summe-Produkt-Algorithmus keine exakte Inferenz mehr möglich (siehe Abschnitt \ref{sec:Loopy-Belief-Propagation}).
Es ist jedoch möglich, das originale Bayessche Netz durch Clustering in eine graphische Struktur zu überführen, auf der Glaubenspropagation mit exakten Ergebnissen möglich ist. Der Transformationsalgorithmus fasst Knoten, die Teil einer Schleife sind, zu Clustern zusammen. Das Ergebnis ist ein baumförmiger Cluster-Graph, der sogenannte Junction Tree, auf welchem anschließend das Message Passing durchgeführt wird. 

Der Junction-Tree-Algorithmus liefert für kleinere Netze sehr gute Ergebnisse, hat aber das Problem, dass seine Komplexität mit der maximalen Anzahl von Variablen in einem Cluster exponentiell ansteigt, was ihn für große komplexe Netze ungeeignet macht. Für die in dieser Arbeit behandelte Problemstellung ist er geeignet, was bereits in \cite{beleg} gezeigt wurde, wo in Kapitel 2.5 auch eine detaillierte Beschreibung des Algorithmus zu finden ist. Da er in Infer.NET jedoch nicht implementiert ist und eine eigene Implementation den Rahmen dieser Arbeit gesprengt hätte, wird im praktischen Teil eine Variante der Glaubenspropagation verwendet, die im folgenden Abschnitt beschrieben wird.

\begin{figure}[ht!]
\centering
\begin{tikzpicture}[every label/.style={font=\small}]
\tikzstyle{cluster}=[draw, font=\small, rounded corners=5pt, inner sep=10pt]
\tikzstyle{sepset}=[draw, font=\scriptsize, inner sep=5pt]
\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]
\tikzstyle{phantom}=[vertex,draw=none]
\tikzstyle{dots}=[loosely dotted,shorten <=3pt, shorten >=3pt]
\tikzstyle{message}=[above, inner sep=10pt,font=\footnotesize]
\tikzstyle{message arrow}=[->,>=stealth,
     shorten >=10pt, shorten <=10pt,
     decoration={sl,raise=8pt},decorate,sloped]

\node[cluster] at (0,0) (DAH)          {$D,A,H$};
\node[sepset,  right=1.5 of DAH] (AH)    {$A,H$};
\node[cluster, right=1.5 of AH] (AHI) {$A,H,I$};
\node[sepset,  right=1.5 of AHI] (A)   {$A$};
\node[cluster, right=1.5 of A] (AS)  {$A,S$};
\path
      (DAH) edge (AH)
      (AH) edge (AHI)
      (AHI) edge (A)
      (A) edge (AS)
      ;
\end{tikzpicture}
\caption{Cluster-Graph für das Netz aus Abbildung \ref{Karzinomnetz}.}
\label{fig:cluster_graph}
\end{figure}

\subsubsection{Approximative Inferenz mit Loopy Belief Propagation}
\label{sec:Loopy-Belief-Propagation}
Der Summe-Produkt-Algorithmus kann auch auf Faktorgraphen mit Schleifen angewandt werden. Diese sogenannte Loopy Belief Propagation (LBP) ist ein iteratives Verfahren, bei dem die Glaubenspropagation bis zum Erreichen eines Konvergenzkriteriums wiederholt wird (Algorithmus \ref{alg:loopy_belief_propagation}). Die Ergebnisse sind jetzt jedoch nicht mehr exakt, sondern eine Näherung.

\begin{algorithm}[H]
\begin{algorithmic}[1]
\Function{LBP}{}
\ForAll{Kanten zwischen Faktoren $f$ und Variablen $X$}
  \State Initialisiere $\mu_{f\rightarrow X}^{(0)}$ und $\mu_{X\rightarrow f}^{(0)}$ mit Gleichverteilung
\EndFor
\While{$\mu^{(t+1)} \neq \mu^{(t)}$} \Comment Muss für jede Nachricht $\mu$ überprüft werden
  \ForAll{Kanten zwischen Faktoren $f$ und Variablen $X$}
    \State $\mu_{f\rightarrow X}^{(t+1)}\leftarrow$\Call{CalcFactorMessage}{$\mu_{X_j \in \mathcal N(f)\backslash X\rightarrow f}^{(t)}$}\Comment{Gleichung \ref{eq:LMP_update_1}}
    \State $\mu_{X\rightarrow f}^{(t+1)}\leftarrow$\Call{CalcNodeMessage}{$\mu_{f_i\in\mathcal N(X)\backslash f\rightarrow X}^{(t)}$}\Comment{Gleichung \ref{eq:LMP_update_2}}
    \State $t \gets t+1$
  \EndFor
\EndWhile
\EndFunction 
\end{algorithmic}
\caption{Loopy Belief Propagation}
\label{alg:loopy_belief_propagation}
\end{algorithm}

Das Prinzip eines Iterationsschrittes ist das gleiche wie beim vollständigen Message-Passing-Schema aus Abschnitt \ref{sec:message_passing_on_factor_graphs}: Durch jede Kante des Graphen wird in beide Richtungen je eine Nachricht geschickt. Der Unterschied ist, dass bei Loopy Belief Propagation zur Berechnung einer Nachricht die Nachrichten aus dem vorhergehenden Iterationsschritt verwendet werden, während bei der normalen Glaubenspropagation die Berechnung einer Nachricht auf Nachrichten desselben Iterationsschrittes basiert (es gibt ja nur den einen). Sei $t$ der vorhergehende Iterationsschritt und $t+1$ der aktuelle Iterationsschritt, so berechnen sich die Nachrichten in Schritt $t+1$ wie folgt:
\begin{align}
\label{eq:LMP_update_1}
\mu_{f\rightarrow X}^{(t+1)}(X)&= \sum_{X_1}\cdots\sum_{X_m}f_s(X,X_1,\dots,X_m) \prod_{X_j\in \mathcal N(f)\backslash X} \mu_{X_j\rightarrow f}^{(t)}(X_j)\\
\mu_{X\rightarrow f}^{(t+1)}(X)&=\prod_{f_i\in\mathcal N(X)\backslash f} \mu_{f_i\rightarrow X}^{(t)}(X)
\label{eq:LMP_update_2}
\end{align}
wobei $\mu_{f\rightarrow X}^{(t+1)}(X)$ die Faktornachrichten und $\mu_{X\rightarrow f}^{(t+1)}(X)$ die Knotennachrichten sind.

Damit die Nachrichten für Schritt $t=1$ berechnet werden können, müssen sie für alle Kanten für Schritt $t=0$ initialisiert werden. Da die Nachrichten selbst Wahrscheinlichkeitsverteilungen sind, werden sie typischerweise mit einer Gleichverteilung initialisiert. Danach werden mit jedem Iterationsschritt alle Nachrichten mit den Gleichungen \ref{eq:LMP_update_1} bzw. \ref{eq:LMP_update_2} aktualisiert. Es wird solange iteriert, bis die Nachrichten konvergieren, also für alle Nachrichten $\mu$
$$\mu^{(t+1)}=\mu^{(t)}$$
gilt oder ein anderes Abbruchkriterium (z.B. eine maximale Zahl von Iterationen) erreicht ist.
Denn es ist nicht garantiert, dass die Nachrichten konvergieren. In bestimmten Fällen ist es möglich, dass die Nachrichten ab einer gewissen Iteration oszillieren. Es hat sich gezeigt, dass die Reihenfolge, in der die Nachrichten in einem Iterationsschritt neu berechnet werden, die Konvergenz beeinflusst. Ein gleichzeitiges Aktualisieren der Nachrichten führt deutlich häufiger zum Oszillieren als das Nacheinander-Berechnen. Ein geschicktes Planen der Reihenfolge, in der die Nachrichten berechnet werden, verbessert die Ergebnisse auch bezüglich ihrer Genauigkeit weiter. Für dieses Scheduling der Aktualisierungsreihenfolge gibt es verschiedene Verfahren, wovon einige in \cite{Sutton_McCallum_Dynamic_Schedules_BP} beschrieben werden. Eine Analyse, unter welchen Bedingungen LBP konvergiert, findet sich in \cite{Mooij_Kappen_Sufficient_Condidtions_Convergence_SPA}.

% Zunächst werden die Nachrichten $\mu^{(0)}$ für alle Kanten in beide Richtungen initialisiert, typischerweise mit einer Gleichverteilung. Anschließend werden sie iterativ mit den Gleichungen \eqref{eq:LMP_update_1} und \eqref{eq:LMP_update_2} aktualisiert, wobei die Nachrichten für den Iterationsschritt $t+1$ aus denen des vorhergehenden Schrittes $t$ berechnet werden, bis das Konvergenzkriterium 
% $ \mu^{(t+1)}=\mu^{(t)}$ für alle Nachrichten $\mu$ erreicht ist. \todo{plausibler formulieren, evtl. Pseudocode}
% Die Nachrichten werden so lange durch den Graphen propagiert, bis sie konvergieren. 
Obwohl der Algorithmus keine Konvergenz garantiert, so hat er sich doch in sehr vielen Anwendungsfällen bewährt\footnote{Einer der bekanntesten Anwendungsfälle von Loopy Belief Propagation sind die Turbo-Codes, welche erstmals Informationskodierung nahe der Shannongrenze ermöglichten. Sie waren gleichzeitig der Beweis der praktischen Anwendbarkeit des Verfahrens.\cite{Turbo-Codes}} und liefert auch für die in dieser Arbeit beschriebene Art von Bayesschen Netzen sehr gute Ergebnisse.
 LBP ist in Infer.NET in Form von Expectation Propagation \cite{Minka:2001:EPA:647235.720257} implementiert und wird für den praktischen Teil dieser Arbeit verwendet.

\subsection{Approximative Inferenz durch Sampling}
\label{sec:approx_inference}
Ein weiteres Prinzip approximativer Inferenz ist das Erzeugen von Stichproben anhand der im Netz modellierten lokalen Wahrscheinlichkeitsverteilungen. Die relative Häufigkeit der erzeugten Werte ergibt eine Annäherung an die Wahrscheinlichkeit. Je größer die Stichprobe, desto genauer ist der berechnete Wert.
\begin{itemize}
 \item \tbf{Direktes Sampling} erzeugt die Stichproben anhand der Wahrscheinlichkeitsverteilungen in topologischer Reihenfolge, also von Eltern- zu Kindknoten. Sei $N$ die Anzahl aller erzeugten Stichproben und $N(\prb{x})$ die Anzahl der Stichproben, welche mit dem gesuchten spezifischen Ereignis $\prb{x}$ konsistent sind, so ergibt sich die approximierte Wahrscheinlichkeit dieses Ereignisses mit:
 $$\hat{P}(\prb{x}) = \frac{N(\prb{x})}{N} \approx P(\prb{x}).$$
 Dieser naive Ansatz kann keine Evidenz behandeln.
 \item \tbf{Ablehnungssampling} kann Verteilungsapproximationen der Form $\hat{\prb{P}}(x|\prb{e})$ liefern, indem es nur die Stichproben verwendet, die auch mit der beobachteten Evidenz \tbf{e} konsistent sind. Es werden aber viele Stichproben zurückgewiesen, so dass es ziemlich ineffizient ist. Die Wahrscheinlichkeitsverteilung einer Variablen wird wie folgt approximiert:
 $$\hat{\prb{P}}(X|\prb{e}) = \frac{\prb{N}(X,\prb{e})}{N(e)} \approx \prb{P}(X|\prb{e}).$$ 
 \item \tbf{Wahrscheinlichkeitsgewichtung} ist effizienter als Ablehnungssampling, weil es keine nicht verwendeten Stichproben erzeugt und nur Variablen sampelt, die keine Evidenzvariablen sind. Jedes Sample wird nach der Wahrscheinlichkeit gewichtet, mit dem es der Evidenz entspricht. Höher gewichtete Samples fließen stärker in die Berechnung ein als niedrig gewichtete. Bei steigender Anzahl von Evidenzvariablen verschlechtert sich jedoch die Leistung.
 \item \tbf{MCMC-Algorithmen}\footnote{MCMC steht für \textit{Markov Chain Monte Carlo}. Ein solches Verfahren wird auch \tbf{Markov-Ketten-Simulation} genannt. Die Bezeichnung "`Monte Carlo"' geht auf John von Neumann zurück, der diesen Namen in Anspielung auf die Spielbank im gleichnamigen Stadtteil von Monaco vorschlug.\cite{Monte_Carlo}} erzeugen nicht jede einzelne Stichprobe von Grund auf neu, sondern durch zufällige Änderungen an der vorherigen Stichprobe. Der \textit{aktuellen Zustand} spezifiziert für jede Variable einen Wert, der \textit{nächste Zustand} wird vom MCMC-Algorithmus generiert, indem er den aktuellen Zustand zufällig ändert. Ein viel verwendeter Algorithmus ist das \tbf{Gibbs Sampling}, welches sich besonders gut für Bayessche Netze eignet. Der Anfangszustand der Nicht-Evidenz-Variablen wird zufällig festgelegt, anschließend werden diese gesampelt. Das Sampling einer Variablen erfolgt auf Basis der bekannten aktuellen Werte seiner Markov-Decken-Variablen und das Ändern einer Variable entspricht einem Schritt im Zustandsraum und somit einer Stichprobe. Gibbs Sampling ist in Infer.NET implementiert und kann als Inferenz-Algorithmus verwendet werden. Ein Nachteil ist, dass es sehr berechnungsintensiv ist, wenn man hinreichende Genauigkeit erreichen möchte. Außerdem ist es schwer, festzustellen, wann der Algorithmus konvergiert \textendash\ jede zusätzliche Iteration kann das Ergebnis potentiell wieder verschlechtern.
\end{itemize}
\begin{easylist}
\end{easylist}

\subsection{Approximative Inferenz mit Variational Message Passing}
\label{chapter:theory:sec:inference:subsec:VMP}
In Modellen mit vielen kontinuierlichen Variablen oder diskreten Variablen mit vielen Zuständen werden die bedingten Wahrscheinlichkeitsverteilungen zwischen den einzelnen Variablen sehr komplex. Die zur Ermittlung der Wahrscheinlichkeiten nötigen hochdimensionalen Summen und Integrale sind analytisch nicht zu bestimmen und eine numerische Lösung oder Abschätzung durch MCMC-Sampling ist sehr berechnungsintensiv. Für solche Problemstellungen wurde die Methode der Variationsinferenz entwickelt. Dabei wird iterativ sowohl eine Approximation der Modellevidenz $P(\prb V)$ als auch die Posteriori-Verteilung $P(\prb H|\prb V)$ optimiert, wobei $\prb V$ die beobachteten (\textit{visible}) Variablen des Modells und $\prb H$ die verborgenen (\textit{hidden}) Variablen sind.

Die Kernidee ist eine Dekomposition der logarithmierten Modellevidenz:
$$\text{ln }P(\prb V)=\mathcal L(Q) + \text{KL}(Q(\prb H)\parallel P(\prb H|\prb V))).$$
KL$(Q\parallel P)$ ist dabei die Kullback-Leibler-Divergenz, ein Maß für den Unterschied zwischen wahrer Verteilung $P$ und approximierter Verteilung $Q$. $\mathcal L(Q)$ ist eine untere Schranke bezüglich ln $P(\prb V)$, auch als \textit{Freie Energie} bezeichnet, und ist definiert durch
$$\mathcal L(Q) = \left<\text{ln }P(\prb V)\right>_Q - \text{KL}(Q(\prb H)\parallel P(\prb H|\prb V)),$$ wobei die Schätzung $\left<.\right>_Q$ mittels $Q$ erfolgt. Durch Ermittlung des $Q$s, welches die Funktion $\mathcal L(Q)$ maximiert, minimiert man indirekt die Kullback-Leibler-Divergenz zwischen $Q(\prb H)$ und der exakten Posteriori-Verteilung $P(\prb H|\prb V)$. Das heißt, wenn $Q(\prb H)= P(\prb H|\prb V)$ ist, dann ist $\mathcal L(Q)=\text{ln }P(\prb V)$.
Die Optimierung von $\mathcal L(Q)$ erfolgt nun, indem man vereinfachende Beschränkungen bezüglich der funktionalen Form von $Q$ vornimmt. Zunächst sollte $Q$ eine faktorisierbare Wahrscheinlichkeitsverteilung mit
$$Q(\prb H) = \prod_i Q_i(H_i)$$
sein, wobei die einzelnen $Q_i$s eine Posterior-Verteilung von unabhängigen Gruppen von Variablen $\prb H_i$ approximieren, während $\mathcal L(Q)$ die Log-Evidenz ln $P(\prb V)$ approximiert. Des Weiteren sind die einzelnen $Q_i$s aus einer bestimmten Verteilungsfamilie, einer sogenannten Exponentialfamilie, zu wählen. Mitglieder einer Exponentialfamilie lassen sich mittels eines natürlichen Parametervektors $\phi$, eines suffizienten Statistikvektors $\prb u$\footnote{Eine suffiziente Statistik ist eine Stichprobe, aus der sich die zugrundeliegende Verteilung vollständig ableiten lässt.} und eines Normierungsfaktors $g$ bilden: 
$$P(\prb X|\prb Y)=\text{exp}\left[\phi(\prb Y)^\text{T}\prb u(\prb X) + f(\prb X) + g(\prb Y)\right].$$
Innerhalb einer Exponentialfamilie haben die Parameter- und Statistik-Vektoren jeweils die gleiche Form. Eine effiziente Optimierung der einzelnen Faktoren erfolgt durch Austausch der Schätzungen dieser Parameter- und Statistikvektoren zwischen den Knoten in Form eines Message-Passing-Schemas. 

Der Vorteil von VMP besteht darin, dass sich auch sehr komplexe Modelle aus diskreten und kontinuierlichen Verteilungen effizient approximieren lassen. Der Nachteil besteht darin, dass die Approximation nicht beliebig genau werden kann. Bei beobachteten diskreten Variablen mit mehr als zwei Zuständen entspricht die Approximation aufgrund der funktionalen Beschränkung der $Q_i$s nicht der exakten Verteilung. Dies kann bei kleinen, rein diskreten Modellen dazu führen, dass sich dieser Fehler so weit fortpflanzt, dass der Algorithmus schlechtere Ergebnisse liefert als andere Inferenzalgorithmen, die bei geringer Modellgröße und hauptsächlich binären Variablen berechnungstechnisch noch gut handhabbar sind und genauer approximieren können. Wie sich das in der Praxis auswirkt, wird in Abschnitt \ref{chapter:implementation:sec:results:subsec:vmp} beschrieben.

\begin{table}[!htbp]
\footnotesize
\centering
{\renewcommand{\arraystretch}{1.3}
\begin{tabulary}{1.0\textwidth,\tymin=50pt}{|C||C|C|C|C|C|}
\hline
                             & Deterministisch? & Exaktes Ergebnis? & Konvergiert immer? & Effizient? & In Infer.NET verfügbar? \\ \hline\hline
Variablen\-eliminierung      & Ja   & Ja & Ja & Nein, schon beim Berechnen mehrerer Variablen sehr ineffizient & Nein \\ \hline
Loopy Belief Propagation     & Ja   & Nur in einfach verbundenen Netzen & Nein, aber für viele Anwendungen ausreichend & Ja (für diskrete Netze) & Ja, mit Expectation Propagation\\ \hline 
Join Tree Belief Propagation & Ja   & Ja & Ja & Ja (für diskrete nicht zu komplexe Netze) & Nein \\ \hline 
Variational Message Passing  & Ja   & Nein & Ja & Ja & Ja \\ \hline
Gibbs Sampling               & Nein & Bei unbegrenzter Anzahl von Iterationsschritten & Ja, aber Konvergenzzeitpunkt ist schwer festzustellen & Für hohe Genauigkeit sehr berechnungsintensiv & Ja \\ \hline
\end{tabulary}}
\caption{Übersicht über die in dieser Arbeit beschriebenen Inferenzalgorithmen für Bayessche Netze}
\label{Uebersicht Inferenzalgorithmen}
\end{table}

==> chapters/graphs/bayes_net_factor_graph_transition_example.tex <==

\usetikzlibrary{arrows, automata,calc,shapes,decorations,decorations.pathreplacing,positioning}
\pgfdeclaredecoration{sl}{initial}{
  \state{initial}[width=\pgfdecoratedpathlength-1sp]{
     \pgfmoveto{\pgfpointorigin}
  }
  \state{final}{
     \pgflineto{\pgfpointorigin}
    }
}

\tikzstyle{e}=[->,shorten >=0.1pt,>=latex]

\tikzstyle{message}=[above,font=\scriptsize, inner sep=13pt]
\tikzstyle{message arrow}=[->,>=stealth,
     shorten >=2pt, shorten <=2pt, 
     decoration={sl,raise=10pt},decorate]
\tikzstyle{vertex}=[circle, draw, font=\scriptsize, inner sep=0pt, minimum size=20pt]
\tikzstyle{factor}=[draw, fill, inner sep=0pt, minimum size=15pt]
\tikzstyle{description}=[decorate,below, inner sep= 30pt, align=left]

\begin{tikzpicture}[every label/.style={font=\small}]
\tikzstyle{vertex}=[circle, draw, font=\scriptsize, inner sep=0pt, minimum size=25pt]

\begin{scope}
\node (A) at (0,0) [label={above left=0 and 0,font=\large:a)}]{
\begin{tikzpicture}
\node[vertex] (g1_x1) at (0,3) [label=above left : $X_1$]{};
\node[vertex] (g1_x2) at (3,3) [label=above right: $X_2$]{};
\node[vertex] (g1_x3) at (1.5,0) [label=below right: $X_3$]{};
\path
	(g1_x1) edge[e] (g1_x3)
    (g1_x2) edge[e] (g1_x3);
\draw[description] (g1_x3) node{$P(X_3|X_2,X_1)P(X_1)P(X_2)$};
\end{tikzpicture}};
\end{scope}

\node[below right=0 and -1.5 of A.north east] (B) [label={above left=0 and 0,font=\large:b)}]{
\begin{tikzpicture}
\begin{scope}
\node[vertex] (g2_x1) at (0,3)   [label=above left : $X_1$]{};
\node[vertex] (g2_x2) at (3,3)   [label=above right: $X_2$]{};
\node[vertex] (g2_x3) at (1.5,0)   [label=below right: $X_3$]{};
\node[factor] (g2_f)  at (1.5,1.6) [label=above      : $f$]{};
\path
	(g2_x1) edge (g2_f)
    (g2_x2) edge (g2_f)
    (g2_x3) edge (g2_f);
\draw[description] (g2_x3) node{$f(X_1,X_2,X_3)=P(X_3|X_2,X_1)P(X_1)P(X_2)$};
\end{scope}
\end{tikzpicture}};

\node[below right=0 and -1.5 of B.north east] (C) [label={above left=0 and 0,font=\large:c)}]{
\begin{tikzpicture}
\node[vertex] (g3_x1) at (0,3)     [label=above left : $X_1$]{};
\node[vertex] (g3_x2) at (3,3)     [label=above right: $X_2$]{};
\node[vertex] (g3_x3) at (1.5,0)   [label=below right: $X_3$]{};
\node[factor] (g3_fa) at (0,1.6)   [label=left       : $f_a$]{};
\node[factor] (g3_fb) at (3,1.6)   [label=right      : $f_b$]{};
\node[factor] (g3_fc) at (1.5,1.6) [label=above      : $f_c$]{};
\path
	(g3_x1) edge (g3_fa)
    (g3_x2) edge (g3_fb)
	(g3_x1) edge (g3_fc)
    (g3_x2) edge (g3_fc)
    (g3_x3) edge (g3_fc);
\draw[description] (g3_x3) node{$f_c(X_1,X_2,X_3)=P(X_3|X_2,X_1)$\\
$f_a(X_1)=P(X_1)$\\
$f_b(X_2)=P(X_2)$};
\end{tikzpicture}
};
\end{tikzpicture}


==> chapters/tables/RoundedSymptomProbabilityComparisonByAlgorithm.tex <==
{\renewcommand{\arraystretch}{1.1}
\scriptsize
\begin{longtable}{llcrrr}
\hline
\multicolumn{6}{c}{Verteilung der Wertzuweisungen für die beobachteten Variablen der generierten Beispiele}\\* \hline
Merkmal & Diagnose & Wert & JTBP & EP & VMP  \\* \hline \endhead
Anorexia & BrainTumor & 1 & 0 & 0 & 0 \\*
AuraSymptoms & BrainTumor & 1 & 0 & 0 & 0 \\*
BloodCalcium & BrainTumor & 1 & 22 & 22 & 22 \\*
CancerMetastasis & BrainTumor & 1 & 4 & 4 & 4 \\*
Coma & BrainTumor & 1 & 80 & 80 & 80 \\*
IpsilateralConjunctivalInjection & BrainTumor & 1 & 1 & 1 & 1 \\*
IpsilateralLacrimination & BrainTumor & 1 & 1 & 1 & 1 \\*
IpsilateralPtosis & BrainTumor & 1 & 1 & 1 & 1 \\*
Nausea & BrainTumor & 1 & 0 & 0 & 0 \\*
PainDuration & BrainTumor & 0 & 14 & 0 & 0 \\*
PainDuration & BrainTumor & 1 & 13 & 1 & 1 \\*
PainDuration & BrainTumor & 2 & 23 & 2 & 2 \\*
PainDuration & BrainTumor & 3 & 13 & 7 & 7 \\*
PainDuration & BrainTumor & 4 & 13 & 34 & 34 \\*
PainDuration & BrainTumor & 5 & 23 & 57 & 57 \\*
PainIntensityAvrg & BrainTumor & 0 & 12 & 0 & 0 \\*
PainIntensityAvrg & BrainTumor & 1 & 7 & 1 & 1 \\*
PainIntensityAvrg & BrainTumor & 2 & 7 & 3 & 3 \\*
PainIntensityAvrg & BrainTumor & 3 & 14 & 9 & 9 \\*
PainIntensityAvrg & BrainTumor & 4 & 11 & 12 & 12 \\*
PainIntensityAvrg & BrainTumor & 5 & 14 & 10 & 10 \\*
PainIntensityAvrg & BrainTumor & 6 & 7 & 12 & 12 \\*
PainIntensityAvrg & BrainTumor & 7 & 7 & 15 & 15 \\*
PainIntensityAvrg & BrainTumor & 8 & 12 & 17 & 17 \\*
PainIntensityAvrg & BrainTumor & 9 & 7 & 20 & 20 \\*
PainQuality & BrainTumor & 0 & 14 & 0 & 0 \\*
PainQuality & BrainTumor & 1 & 14 & 2 & 2 \\*
PainQuality & BrainTumor & 2 & 14 & 4 & 4 \\*
PainQuality & BrainTumor & 3 & 57 & 94 & 94 \\*
Phonophobia & BrainTumor & 1 & 0 & 0 & 0 \\*
Photophobia & BrainTumor & 1 & 0 & 0 & 0 \\*
Restlessness & BrainTumor & 1 & 1 & 1 & 1 \\*
Sex & BrainTumor & 1 & 54 & 55 & 55 \\*
TriggerAlcohol & BrainTumor & 1 & 0 & 0 & 0 \\*
TriggerAnxiety & BrainTumor & 1 & 1 & 1 & 1 \\*
TriggerBodyStress & BrainTumor & 1 & 1 & 1 & 1 \\*
TriggerDepression & BrainTumor & 1 & 1 & 1 & 1 \\*
TriggerMenstruation & BrainTumor & 1 & 0 & 0 & 0 \\*
TriggerMentalStress & BrainTumor & 1 & 0 & 0 & 0 \\*
TriggerSmoking & BrainTumor & 1 & 0 & 0 & 0 \\*
TriggerUpset & BrainTumor & 1 & 1 & 1 & 1 \\*
TriggerWeatherChange & BrainTumor & 1 & 0 & 0 & 0 \\*
Vomiting & BrainTumor & 1 & 0 & 0 & 0 \\
Anorexia & ClusterHeadache & 1 & 0 & 0 & 0 \\*
AuraSymptoms & ClusterHeadache & 1 & 10 & 10 & 10 \\*
BloodCalcium & ClusterHeadache & 1 & 21 & 21 & 21 \\*
CancerMetastasis & ClusterHeadache & 1 & 1 & 1 & 1 \\*
Coma & ClusterHeadache & 1 & 20 & 20 & 20 \\*
IpsilateralConjunctivalInjection & ClusterHeadache & 1 & 74 & 74 & 74 \\*
IpsilateralLacrimination & ClusterHeadache & 1 & 93 & 93 & 93 \\*
IpsilateralPtosis & ClusterHeadache & 1 & 68 & 68 & 68 \\*
Nausea & ClusterHeadache & 1 & 50 & 50 & 50 \\*
PainDuration & ClusterHeadache & 0 & 23 & 1 & 1 \\*
PainDuration & ClusterHeadache & 1 & 19 & 7 & 7 \\*
PainDuration & ClusterHeadache & 2 & 12 & 16 & 16 \\*
PainDuration & ClusterHeadache & 3 & 12 & 18 & 18 \\*
PainDuration & ClusterHeadache & 4 & 21 & 25 & 25 \\*
PainDuration & ClusterHeadache & 5 & 12 & 33 & 33 \\*
PainIntensityAvrg & ClusterHeadache & 0 & 11 & 0 & 0 \\*
PainIntensityAvrg & ClusterHeadache & 1 & 7 & 1 & 1 \\*
PainIntensityAvrg & ClusterHeadache & 2 & 7 & 2 & 2 \\*
PainIntensityAvrg & ClusterHeadache & 3 & 17 & 11 & 11 \\*
PainIntensityAvrg & ClusterHeadache & 4 & 15 & 16 & 16 \\*
PainIntensityAvrg & ClusterHeadache & 5 & 13 & 10 & 10 \\*
PainIntensityAvrg & ClusterHeadache & 6 & 7 & 12 & 12 \\*
PainIntensityAvrg & ClusterHeadache & 7 & 7 & 14 & 14 \\*
PainIntensityAvrg & ClusterHeadache & 8 & 11 & 16 & 16 \\*
PainIntensityAvrg & ClusterHeadache & 9 & 7 & 19 & 19 \\*
PainQuality & ClusterHeadache & 0 & 10 & 0 & 0 \\*
PainQuality & ClusterHeadache & 1 & 10 & 1 & 1 \\*
PainQuality & ClusterHeadache & 2 & 10 & 2 & 2 \\*
PainQuality & ClusterHeadache & 3 & 70 & 97 & 97 \\*
Phonophobia & ClusterHeadache & 1 & 43 & 43 & 43 \\*
Photophobia & ClusterHeadache & 1 & 56 & 54 & 54 \\*
Restlessness & ClusterHeadache & 1 & 80 & 80 & 80 \\*
Sex & ClusterHeadache & 1 & 78 & 79 & 79 \\*
TriggerAlcohol & ClusterHeadache & 1 & 20 & 20 & 20 \\*
TriggerAnxiety & ClusterHeadache & 1 & 1 & 1 & 1 \\*
TriggerBodyStress & ClusterHeadache & 1 & 1 & 1 & 1 \\*
TriggerDepression & ClusterHeadache & 1 & 1 & 1 & 1 \\*
TriggerMenstruation & ClusterHeadache & 1 & 0 & 0 & 0 \\*
TriggerMentalStress & ClusterHeadache & 1 & 0 & 0 & 0 \\*
TriggerSmoking & ClusterHeadache & 1 & 20 & 20 & 20 \\*
TriggerUpset & ClusterHeadache & 1 & 1 & 1 & 1 \\*
TriggerWeatherChange & ClusterHeadache & 1 & 0 & 0 & 0 \\*
Vomiting & ClusterHeadache & 1 & 0 & 0 & 0 \\
Anorexia & MigraineWithAura & 1 & 82 & 82 & 82 \\*
AuraSymptoms & MigraineWithAura & 1 & 95 & 95 & 95 \\*
BloodCalcium & MigraineWithAura & 1 & 21 & 21 & 21 \\*
CancerMetastasis & MigraineWithAura & 1 & 1 & 1 & 1 \\*
Coma & MigraineWithAura & 1 & 20 & 20 & 20 \\*
IpsilateralConjunctivalInjection & MigraineWithAura & 1 & 1 & 1 & 1 \\*
IpsilateralLacrimination & MigraineWithAura & 1 & 1 & 1 & 1 \\*
IpsilateralPtosis & MigraineWithAura & 1 & 1 & 1 & 1 \\*
Nausea & MigraineWithAura & 1 & 82 & 82 & 82 \\*
PainDuration & MigraineWithAura & 0 & 23 & 1 & 1 \\*
PainDuration & MigraineWithAura & 1 & 21 & 8 & 8 \\*
PainDuration & MigraineWithAura & 2 & 13 & 15 & 15 \\*
PainDuration & MigraineWithAura & 3 & 13 & 18 & 18 \\*
PainDuration & MigraineWithAura & 4 & 19 & 25 & 25 \\*
PainDuration & MigraineWithAura & 5 & 13 & 33 & 33 \\*
PainIntensityAvrg & MigraineWithAura & 0 & 16 & 0 & 0 \\*
PainIntensityAvrg & MigraineWithAura & 1 & 8 & 0 & 0 \\*
PainIntensityAvrg & MigraineWithAura & 2 & 8 & 3 & 3 \\*
PainIntensityAvrg & MigraineWithAura & 3 & 17 & 9 & 9 \\*
PainIntensityAvrg & MigraineWithAura & 4 & 12 & 11 & 11 \\*
PainIntensityAvrg & MigraineWithAura & 5 & 9 & 10 & 10 \\*
PainIntensityAvrg & MigraineWithAura & 6 & 8 & 12 & 12 \\*
PainIntensityAvrg & MigraineWithAura & 7 & 8 & 15 & 15 \\*
PainIntensityAvrg & MigraineWithAura & 8 & 7 & 18 & 18 \\*
PainIntensityAvrg & MigraineWithAura & 9 & 8 & 22 & 22 \\*
PainQuality & MigraineWithAura & 0 & 37 & 2 & 2 \\*
PainQuality & MigraineWithAura & 1 & 12 & 7 & 7 \\*
PainQuality & MigraineWithAura & 2 & 17 & 12 & 12 \\*
PainQuality & MigraineWithAura & 3 & 34 & 79 & 79 \\*
Phonophobia & MigraineWithAura & 1 & 87 & 87 & 87 \\*
Photophobia & MigraineWithAura & 1 & 80 & 80 & 80 \\*
Restlessness & MigraineWithAura & 1 & 1 & 1 & 1 \\*
Sex & MigraineWithAura & 1 & 32 & 34 & 34 \\*
TriggerAlcohol & MigraineWithAura & 1 & 8 & 8 & 8 \\*
TriggerAnxiety & MigraineWithAura & 1 & 1 & 1 & 1 \\*
TriggerBodyStress & MigraineWithAura & 1 & 1 & 1 & 1 \\*
TriggerDepression & MigraineWithAura & 1 & 1 & 1 & 1 \\*
TriggerMenstruation & MigraineWithAura & 1 & 11 & 11 & 11 \\*
TriggerMentalStress & MigraineWithAura & 1 & 37 & 37 & 37 \\*
TriggerSmoking & MigraineWithAura & 1 & 3 & 3 & 3 \\*
TriggerUpset & MigraineWithAura & 1 & 1 & 1 & 1 \\*
TriggerWeatherChange & MigraineWithAura & 1 & 18 & 17 & 17 \\*
Vomiting & MigraineWithAura & 1 & 52 & 52 & 52 \\
Anorexia & MigraineWithoutAura & 1 & 82 & 82 & 82 \\*
AuraSymptoms & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
BloodCalcium & MigraineWithoutAura & 1 & 21 & 21 & 21 \\*
CancerMetastasis & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
Coma & MigraineWithoutAura & 1 & 20 & 20 & 20 \\*
IpsilateralConjunctivalInjection & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
IpsilateralLacrimination & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
IpsilateralPtosis & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
Nausea & MigraineWithoutAura & 1 & 82 & 82 & 82 \\*
PainDuration & MigraineWithoutAura & 0 & 23 & 1 & 1 \\*
PainDuration & MigraineWithoutAura & 1 & 21 & 8 & 8 \\*
PainDuration & MigraineWithoutAura & 2 & 13 & 15 & 15 \\*
PainDuration & MigraineWithoutAura & 3 & 13 & 18 & 18 \\*
PainDuration & MigraineWithoutAura & 4 & 19 & 25 & 25 \\*
PainDuration & MigraineWithoutAura & 5 & 13 & 33 & 33 \\*
PainIntensityAvrg & MigraineWithoutAura & 0 & 16 & 0 & 0 \\*
PainIntensityAvrg & MigraineWithoutAura & 1 & 8 & 0 & 0 \\*
PainIntensityAvrg & MigraineWithoutAura & 2 & 8 & 3 & 3 \\*
PainIntensityAvrg & MigraineWithoutAura & 3 & 17 & 9 & 9 \\*
PainIntensityAvrg & MigraineWithoutAura & 4 & 12 & 11 & 11 \\*
PainIntensityAvrg & MigraineWithoutAura & 5 & 9 & 10 & 10 \\*
PainIntensityAvrg & MigraineWithoutAura & 6 & 8 & 12 & 12 \\*
PainIntensityAvrg & MigraineWithoutAura & 7 & 8 & 15 & 15 \\*
PainIntensityAvrg & MigraineWithoutAura & 8 & 7 & 18 & 18 \\*
PainIntensityAvrg & MigraineWithoutAura & 9 & 8 & 22 & 22 \\*
PainQuality & MigraineWithoutAura & 0 & 37 & 2 & 2 \\*
PainQuality & MigraineWithoutAura & 1 & 12 & 7 & 7 \\*
PainQuality & MigraineWithoutAura & 2 & 17 & 12 & 12 \\*
PainQuality & MigraineWithoutAura & 3 & 34 & 79 & 79 \\*
Phonophobia & MigraineWithoutAura & 1 & 98 & 98 & 98 \\*
Photophobia & MigraineWithoutAura & 1 & 94 & 94 & 94 \\*
Restlessness & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
Sex & MigraineWithoutAura & 1 & 13 & 13 & 13 \\*
TriggerAlcohol & MigraineWithoutAura & 1 & 28 & 28 & 28 \\*
TriggerAnxiety & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
TriggerBodyStress & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
TriggerDepression & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
TriggerMenstruation & MigraineWithoutAura & 1 & 26 & 26 & 26 \\*
TriggerMentalStress & MigraineWithoutAura & 1 & 43 & 43 & 43 \\*
TriggerSmoking & MigraineWithoutAura & 1 & 10 & 10 & 10 \\*
TriggerUpset & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
TriggerWeatherChange & MigraineWithoutAura & 1 & 25 & 25 & 25 \\*
Vomiting & MigraineWithoutAura & 1 & 62 & 62 & 62 \\
Anorexia & TensionHeadache & 1 & 18 & 18 & 18 \\*
AuraSymptoms & TensionHeadache & 1 & 0 & 0 & 0 \\*
BloodCalcium & TensionHeadache & 1 & 21 & 21 & 21 \\*
CancerMetastasis & TensionHeadache & 1 & 1 & 1 & 1 \\*
Coma & TensionHeadache & 1 & 20 & 20 & 20 \\*
IpsilateralConjunctivalInjection & TensionHeadache & 1 & 1 & 1 & 1 \\*
IpsilateralLacrimination & TensionHeadache & 1 & 1 & 1 & 1 \\*
IpsilateralPtosis & TensionHeadache & 1 & 1 & 1 & 1 \\*
Nausea & TensionHeadache & 1 & 4 & 4 & 4 \\*
PainDuration & TensionHeadache & 0 & 21 & 1 & 1 \\*
PainDuration & TensionHeadache & 1 & 19 & 6 & 6 \\*
PainDuration & TensionHeadache & 2 & 13 & 15 & 15 \\*
PainDuration & TensionHeadache & 3 & 13 & 18 & 18 \\*
PainDuration & TensionHeadache & 4 & 19 & 26 & 26 \\*
PainDuration & TensionHeadache & 5 & 13 & 35 & 35 \\*
PainIntensityAvrg & TensionHeadache & 0 & 21 & 0 & 0 \\*
PainIntensityAvrg & TensionHeadache & 1 & 5 & 2 & 2 \\*
PainIntensityAvrg & TensionHeadache & 2 & 5 & 6 & 6 \\*
PainIntensityAvrg & TensionHeadache & 3 & 12 & 14 & 14 \\*
PainIntensityAvrg & TensionHeadache & 4 & 9 & 15 & 15 \\*
PainIntensityAvrg & TensionHeadache & 5 & 11 & 10 & 10 \\*
PainIntensityAvrg & TensionHeadache & 6 & 5 & 11 & 11 \\*
PainIntensityAvrg & TensionHeadache & 7 & 5 & 13 & 13 \\*
PainIntensityAvrg & TensionHeadache & 8 & 21 & 14 & 14 \\*
PainIntensityAvrg & TensionHeadache & 9 & 5 & 15 & 15 \\*
PainQuality & TensionHeadache & 0 & 17 & 0 & 0 \\*
PainQuality & TensionHeadache & 1 & 12 & 8 & 8 \\*
PainQuality & TensionHeadache & 2 & 37 & 11 & 11 \\*
PainQuality & TensionHeadache & 3 & 34 & 80 & 80 \\*
Phonophobia & TensionHeadache & 1 & 0 & 0 & 0 \\*
Photophobia & TensionHeadache & 1 & 10 & 10 & 10 \\*
Restlessness & TensionHeadache & 1 & 1 & 1 & 1 \\*
Sex & TensionHeadache & 1 & 43 & 45 & 45 \\*
TriggerAlcohol & TensionHeadache & 1 & 27 & 27 & 27 \\*
TriggerAnxiety & TensionHeadache & 1 & 40 & 40 & 40 \\*
TriggerBodyStress & TensionHeadache & 1 & 40 & 40 & 40 \\*
TriggerDepression & TensionHeadache & 1 & 30 & 30 & 30 \\*
TriggerMenstruation & TensionHeadache & 1 & 23 & 22 & 22 \\*
TriggerMentalStress & TensionHeadache & 1 & 71 & 71 & 71 \\*
TriggerSmoking & TensionHeadache & 1 & 36 & 36 & 36 \\*
TriggerUpset & TensionHeadache & 1 & 30 & 30 & 30 \\*
TriggerWeatherChange & TensionHeadache & 1 & 27 & 27 & 27 \\*
Vomiting & TensionHeadache & 1 & 0 & 0 & 0 \\*
\hline
\caption{Verteilung der Wertzuweisungen für die beobachteten Werte der generierten Beispiele für alle drei Algorithmen und die jeweilige erwartete Diagnose.}
\label{tab:observable_distributions}
\end{longtable}}


==> chapters/tables/RoundedSymptomProbabilityComparisonByAlgorithm_JTBP_Samples.tex <==
% \begin{table}[htbp!]
% \centering
% \small
% \makebox[\textwidth][c]{
% 
{\renewcommand{\arraystretch}{1.1}
\scriptsize
\begin{longtable}{llcrrr}
\hline
\multicolumn{6}{c}{Verteilung der Wertzuweisungen der beobachteten Variablen für die generierten Beispiele}\\* \hline 
Merkmal & Diagnose & Wert & JTBP & EP & VMP  \\* \hline \endhead
Anorexia & BrainTumor & 1 & 0 & 0 & 0 \\*
AuraSymptoms & BrainTumor & 1 & 0 & 50 & 50 \\*
BloodCalcium & BrainTumor & 1 & 22 & 22 & 22 \\*
CancerMetastasis & BrainTumor & 1 & 4 & 4 & 4 \\*
Coma & BrainTumor & 1 & 80 & 80 & 80 \\*
IpsilateralConjunctivalInjection & BrainTumor & 1 & 1 & 1 & 1 \\*
IpsilateralLacrimination & BrainTumor & 1 & 1 & 1 & 1 \\*
IpsilateralPtosis & BrainTumor & 1 & 1 & 1 & 1 \\*
Nausea & BrainTumor & 1 & 0 & 0 & 0 \\*
PainDuration & BrainTumor & 0 & 14 & 0 & 0 \\*
PainDuration & BrainTumor & 1 & 13 & 1 & 1 \\*
PainDuration & BrainTumor & 2 & 23 & 2 & 2 \\*
PainDuration & BrainTumor & 3 & 13 & 7 & 7 \\*
PainDuration & BrainTumor & 4 & 13 & 34 & 34 \\*
PainDuration & BrainTumor & 5 & 23 & 57 & 57 \\*
PainIntensityAvrg & BrainTumor & 0 & 12 & 0 & 0 \\*
PainIntensityAvrg & BrainTumor & 1 & 7 & 1 & 1 \\*
PainIntensityAvrg & BrainTumor & 2 & 7 & 3 & 3 \\*
PainIntensityAvrg & BrainTumor & 3 & 14 & 9 & 9 \\*
PainIntensityAvrg & BrainTumor & 4 & 11 & 12 & 12 \\*
PainIntensityAvrg & BrainTumor & 5 & 14 & 10 & 10 \\*
PainIntensityAvrg & BrainTumor & 6 & 7 & 12 & 12 \\*
PainIntensityAvrg & BrainTumor & 7 & 7 & 15 & 15 \\*
PainIntensityAvrg & BrainTumor & 8 & 12 & 17 & 17 \\*
PainIntensityAvrg & BrainTumor & 9 & 7 & 20 & 20 \\*
PainQuality & BrainTumor & 0 & 14 & 0 & 0 \\*
PainQuality & BrainTumor & 1 & 14 & 2 & 2 \\*
PainQuality & BrainTumor & 2 & 14 & 4 & 4 \\*
PainQuality & BrainTumor & 3 & 57 & 94 & 94 \\*
Phonophobia & BrainTumor & 1 & 0 & 0 & 0 \\*
Photophobia & BrainTumor & 1 & 0 & 0 & 0 \\*
Restlessness & BrainTumor & 1 & 1 & 1 & 1 \\*
Sex & BrainTumor & 1 & 54 & 55 & 55 \\*
TriggerAlcohol & BrainTumor & 1 & 0 & 0 & 0 \\*
TriggerAnxiety & BrainTumor & 1 & 1 & 1 & 1 \\*
TriggerBodyStress & BrainTumor & 1 & 1 & 1 & 1 \\*
TriggerDepression & BrainTumor & 1 & 1 & 1 & 1 \\*
TriggerMenstruation & BrainTumor & 1 & 0 & 0 & 0 \\*
TriggerMentalStress & BrainTumor & 1 & 0 & 0 & 0 \\*
TriggerSmoking & BrainTumor & 1 & 0 & 0 & 0 \\*
TriggerUpset & BrainTumor & 1 & 1 & 1 & 1 \\*
TriggerWeatherChange & BrainTumor & 1 & 0 & 0 & 0 \\*
Vomiting & BrainTumor & 1 & 0 & 0 & 0 \\ 
\pagebreak Anorexia & ClusterHeadache & 1 & 0 & 0 & 0 \\*
AuraSymptoms & ClusterHeadache & 1 & 10 & 60 & 60 \\*
BloodCalcium & ClusterHeadache & 1 & 21 & 21 & 21 \\*
CancerMetastasis & ClusterHeadache & 1 & 1 & 1 & 1 \\*
Coma & ClusterHeadache & 1 & 20 & 20 & 20 \\*
IpsilateralConjunctivalInjection & ClusterHeadache & 1 & 74 & 74 & 74 \\*
IpsilateralLacrimination & ClusterHeadache & 1 & 93 & 93 & 93 \\*
IpsilateralPtosis & ClusterHeadache & 1 & 68 & 68 & 68 \\*
Nausea & ClusterHeadache & 1 & 50 & 50 & 50 \\*
PainDuration & ClusterHeadache & 0 & 23 & 1 & 1 \\*
PainDuration & ClusterHeadache & 1 & 19 & 7 & 7 \\*
PainDuration & ClusterHeadache & 2 & 12 & 16 & 16 \\*
PainDuration & ClusterHeadache & 3 & 12 & 18 & 18 \\*
PainDuration & ClusterHeadache & 4 & 21 & 25 & 25 \\*
PainDuration & ClusterHeadache & 5 & 12 & 33 & 33 \\*
PainIntensityAvrg & ClusterHeadache & 0 & 11 & 0 & 0 \\*
PainIntensityAvrg & ClusterHeadache & 1 & 7 & 1 & 1 \\*
PainIntensityAvrg & ClusterHeadache & 2 & 7 & 2 & 2 \\*
PainIntensityAvrg & ClusterHeadache & 3 & 17 & 11 & 11 \\*
PainIntensityAvrg & ClusterHeadache & 4 & 15 & 16 & 16 \\*
PainIntensityAvrg & ClusterHeadache & 5 & 13 & 10 & 10 \\*
PainIntensityAvrg & ClusterHeadache & 6 & 7 & 12 & 12 \\*
PainIntensityAvrg & ClusterHeadache & 7 & 7 & 14 & 14 \\*
PainIntensityAvrg & ClusterHeadache & 8 & 11 & 16 & 16 \\*
PainIntensityAvrg & ClusterHeadache & 9 & 7 & 19 & 19 \\*
PainQuality & ClusterHeadache & 0 & 10 & 0 & 0 \\*
PainQuality & ClusterHeadache & 1 & 10 & 1 & 1 \\*
PainQuality & ClusterHeadache & 2 & 10 & 2 & 2 \\*
PainQuality & ClusterHeadache & 3 & 70 & 97 & 97 \\*
Phonophobia & ClusterHeadache & 1 & 43 & 43 & 43 \\*
Photophobia & ClusterHeadache & 1 & 56 & 54 & 54 \\*
Restlessness & ClusterHeadache & 1 & 80 & 80 & 80 \\*
Sex & ClusterHeadache & 1 & 78 & 79 & 79 \\*
TriggerAlcohol & ClusterHeadache & 1 & 20 & 20 & 20 \\*
TriggerAnxiety & ClusterHeadache & 1 & 1 & 1 & 1 \\*
TriggerBodyStress & ClusterHeadache & 1 & 1 & 1 & 1 \\*
TriggerDepression & ClusterHeadache & 1 & 1 & 1 & 1 \\*
TriggerMenstruation & ClusterHeadache & 1 & 0 & 0 & 0 \\*
TriggerMentalStress & ClusterHeadache & 1 & 0 & 0 & 0 \\*
TriggerSmoking & ClusterHeadache & 1 & 20 & 20 & 20 \\*
TriggerUpset & ClusterHeadache & 1 & 1 & 1 & 1 \\*
TriggerWeatherChange & ClusterHeadache & 1 & 0 & 0 & 0 \\*
Vomiting & ClusterHeadache & 1 & 0 & 0 & 0 \\
Anorexia & MigraineWithAura & 1 & 82 & 82 & 82 \\*
AuraSymptoms & MigraineWithAura & 1 & 95 & 95 & 95 \\*
BloodCalcium & MigraineWithAura & 1 & 21 & 21 & 21 \\*
CancerMetastasis & MigraineWithAura & 1 & 1 & 1 & 1 \\*
Coma & MigraineWithAura & 1 & 20 & 20 & 20 \\*
IpsilateralConjunctivalInjection & MigraineWithAura & 1 & 1 & 1 & 1 \\*
IpsilateralLacrimination & MigraineWithAura & 1 & 1 & 1 & 1 \\*
IpsilateralPtosis & MigraineWithAura & 1 & 1 & 1 & 1 \\*
Nausea & MigraineWithAura & 1 & 82 & 82 & 82 \\*
PainDuration & MigraineWithAura & 0 & 23 & 1 & 1 \\*
PainDuration & MigraineWithAura & 1 & 21 & 8 & 8 \\*
PainDuration & MigraineWithAura & 2 & 13 & 15 & 15 \\*
PainDuration & MigraineWithAura & 3 & 13 & 18 & 18 \\*
PainDuration & MigraineWithAura & 4 & 19 & 25 & 25 \\*
PainDuration & MigraineWithAura & 5 & 13 & 33 & 33 \\*
PainIntensityAvrg & MigraineWithAura & 0 & 16 & 0 & 0 \\*
PainIntensityAvrg & MigraineWithAura & 1 & 8 & 0 & 0 \\*
PainIntensityAvrg & MigraineWithAura & 2 & 8 & 3 & 3 \\*
PainIntensityAvrg & MigraineWithAura & 3 & 17 & 9 & 9 \\*
PainIntensityAvrg & MigraineWithAura & 4 & 12 & 11 & 11 \\*
PainIntensityAvrg & MigraineWithAura & 5 & 9 & 10 & 10 \\*
PainIntensityAvrg & MigraineWithAura & 6 & 8 & 12 & 12 \\*
PainIntensityAvrg & MigraineWithAura & 7 & 8 & 15 & 15 \\*
PainIntensityAvrg & MigraineWithAura & 8 & 7 & 18 & 18 \\*
PainIntensityAvrg & MigraineWithAura & 9 & 8 & 22 & 22 \\*
PainQuality & MigraineWithAura & 0 & 37 & 2 & 2 \\*
PainQuality & MigraineWithAura & 1 & 12 & 7 & 7 \\*
PainQuality & MigraineWithAura & 2 & 17 & 12 & 12 \\*
PainQuality & MigraineWithAura & 3 & 34 & 79 & 79 \\*
Phonophobia & MigraineWithAura & 1 & 87 & 87 & 87 \\*
Photophobia & MigraineWithAura & 1 & 80 & 80 & 80 \\*
Restlessness & MigraineWithAura & 1 & 1 & 1 & 1 \\*
Sex & MigraineWithAura & 1 & 32 & 34 & 34 \\*
TriggerAlcohol & MigraineWithAura & 1 & 8 & 8 & 8 \\*
TriggerAnxiety & MigraineWithAura & 1 & 1 & 1 & 1 \\*
TriggerBodyStress & MigraineWithAura & 1 & 1 & 1 & 1 \\*
TriggerDepression & MigraineWithAura & 1 & 1 & 1 & 1 \\*
TriggerMenstruation & MigraineWithAura & 1 & 11 & 11 & 11 \\*
TriggerMentalStress & MigraineWithAura & 1 & 37 & 37 & 37 \\*
TriggerSmoking & MigraineWithAura & 1 & 3 & 3 & 3 \\*
TriggerUpset & MigraineWithAura & 1 & 1 & 1 & 1 \\*
TriggerWeatherChange & MigraineWithAura & 1 & 18 & 17 & 17 \\*
Vomiting & MigraineWithAura & 1 & 52 & 52 & 52 \\
Anorexia & MigraineWithoutAura & 1 & 82 & 82 & 82 \\*
AuraSymptoms & MigraineWithoutAura & 1 & 1 & 10 & 10 \\*
BloodCalcium & MigraineWithoutAura & 1 & 21 & 21 & 21 \\*
CancerMetastasis & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
Coma & MigraineWithoutAura & 1 & 20 & 20 & 20 \\*
IpsilateralConjunctivalInjection & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
IpsilateralLacrimination & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
IpsilateralPtosis & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
Nausea & MigraineWithoutAura & 1 & 82 & 82 & 82 \\*
PainDuration & MigraineWithoutAura & 0 & 23 & 1 & 1 \\*
PainDuration & MigraineWithoutAura & 1 & 21 & 8 & 8 \\*
PainDuration & MigraineWithoutAura & 2 & 13 & 15 & 15 \\*
PainDuration & MigraineWithoutAura & 3 & 13 & 18 & 18 \\*
PainDuration & MigraineWithoutAura & 4 & 19 & 25 & 25 \\*
PainDuration & MigraineWithoutAura & 5 & 13 & 33 & 33 \\*
PainIntensityAvrg & MigraineWithoutAura & 0 & 16 & 0 & 0 \\*
PainIntensityAvrg & MigraineWithoutAura & 1 & 8 & 0 & 0 \\*
PainIntensityAvrg & MigraineWithoutAura & 2 & 8 & 3 & 3 \\*
PainIntensityAvrg & MigraineWithoutAura & 3 & 17 & 9 & 9 \\*
PainIntensityAvrg & MigraineWithoutAura & 4 & 12 & 11 & 11 \\*
PainIntensityAvrg & MigraineWithoutAura & 5 & 9 & 10 & 10 \\*
PainIntensityAvrg & MigraineWithoutAura & 6 & 8 & 12 & 12 \\*
PainIntensityAvrg & MigraineWithoutAura & 7 & 8 & 15 & 15 \\*
PainIntensityAvrg & MigraineWithoutAura & 8 & 7 & 18 & 18 \\*
PainIntensityAvrg & MigraineWithoutAura & 9 & 8 & 22 & 22 \\*
PainQuality & MigraineWithoutAura & 0 & 37 & 2 & 2 \\*
PainQuality & MigraineWithoutAura & 1 & 12 & 7 & 7 \\*
PainQuality & MigraineWithoutAura & 2 & 17 & 12 & 12 \\*
PainQuality & MigraineWithoutAura & 3 & 34 & 79 & 79 \\*
Phonophobia & MigraineWithoutAura & 1 & 98 & 98 & 98 \\*
Photophobia & MigraineWithoutAura & 1 & 94 & 94 & 94 \\*
Restlessness & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
Sex & MigraineWithoutAura & 1 & 13 & 13 & 13 \\*
TriggerAlcohol & MigraineWithoutAura & 1 & 28 & 28 & 28 \\*
TriggerAnxiety & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
TriggerBodyStress & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
TriggerDepression & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
TriggerMenstruation & MigraineWithoutAura & 1 & 26 & 26 & 26 \\*
TriggerMentalStress & MigraineWithoutAura & 1 & 43 & 43 & 43 \\*
TriggerSmoking & MigraineWithoutAura & 1 & 10 & 10 & 10 \\*
TriggerUpset & MigraineWithoutAura & 1 & 1 & 1 & 1 \\*
TriggerWeatherChange & MigraineWithoutAura & 1 & 25 & 25 & 25 \\*
Vomiting & MigraineWithoutAura & 1 & 62 & 62 & 62 \\
Anorexia & TensionHeadache & 1 & 18 & 18 & 18 \\*
AuraSymptoms & TensionHeadache & 1 & 0 & 50 & 50 \\*
BloodCalcium & TensionHeadache & 1 & 21 & 21 & 21 \\*
CancerMetastasis & TensionHeadache & 1 & 1 & 1 & 1 \\*
Coma & TensionHeadache & 1 & 20 & 20 & 20 \\*
IpsilateralConjunctivalInjection & TensionHeadache & 1 & 1 & 1 & 1 \\*
IpsilateralLacrimination & TensionHeadache & 1 & 1 & 1 & 1 \\*
IpsilateralPtosis & TensionHeadache & 1 & 1 & 1 & 1 \\*
Nausea & TensionHeadache & 1 & 4 & 4 & 4 \\*
PainDuration & TensionHeadache & 0 & 21 & 1 & 1 \\*
PainDuration & TensionHeadache & 1 & 19 & 6 & 6 \\*
PainDuration & TensionHeadache & 2 & 13 & 15 & 15 \\*
PainDuration & TensionHeadache & 3 & 13 & 18 & 18 \\*
PainDuration & TensionHeadache & 4 & 19 & 26 & 26 \\*
PainDuration & TensionHeadache & 5 & 13 & 35 & 35 \\*
PainIntensityAvrg & TensionHeadache & 0 & 21 & 0 & 0 \\*
PainIntensityAvrg & TensionHeadache & 1 & 5 & 2 & 2 \\*
PainIntensityAvrg & TensionHeadache & 2 & 5 & 6 & 6 \\*
PainIntensityAvrg & TensionHeadache & 3 & 12 & 14 & 14 \\*
PainIntensityAvrg & TensionHeadache & 4 & 9 & 15 & 15 \\*
PainIntensityAvrg & TensionHeadache & 5 & 11 & 10 & 10 \\*
PainIntensityAvrg & TensionHeadache & 6 & 5 & 11 & 11 \\*
PainIntensityAvrg & TensionHeadache & 7 & 5 & 13 & 13 \\*
PainIntensityAvrg & TensionHeadache & 8 & 21 & 14 & 14 \\*
PainIntensityAvrg & TensionHeadache & 9 & 5 & 15 & 15 \\*
PainQuality & TensionHeadache & 0 & 17 & 0 & 0 \\*
PainQuality & TensionHeadache & 1 & 12 & 8 & 8 \\*
PainQuality & TensionHeadache & 2 & 37 & 11 & 11 \\*
PainQuality & TensionHeadache & 3 & 34 & 80 & 80 \\*
Phonophobia & TensionHeadache & 1 & 0 & 0 & 0 \\*
Photophobia & TensionHeadache & 1 & 10 & 10 & 10 \\*
Restlessness & TensionHeadache & 1 & 1 & 1 & 1 \\*
Sex & TensionHeadache & 1 & 43 & 45 & 45 \\*
TriggerAlcohol & TensionHeadache & 1 & 27 & 27 & 27 \\*
TriggerAnxiety & TensionHeadache & 1 & 40 & 40 & 40 \\*
TriggerBodyStress & TensionHeadache & 1 & 40 & 40 & 40 \\*
TriggerDepression & TensionHeadache & 1 & 30 & 30 & 30 \\*
TriggerMenstruation & TensionHeadache & 1 & 23 & 22 & 22 \\*
TriggerMentalStress & TensionHeadache & 1 & 71 & 71 & 71 \\*
TriggerSmoking & TensionHeadache & 1 & 36 & 36 & 36 \\*
TriggerUpset & TensionHeadache & 1 & 30 & 30 & 30 \\*
TriggerWeatherChange & TensionHeadache & 1 & 27 & 27 & 27 \\*
Vomiting & TensionHeadache & 1 & 0 & 0 & 0 \\*
\hline
\caption{Verteilung der Wertzuweisungen für die beobachteten Werte der generierten Beispiele für alle drei Algorithmen und die jeweilige erwartete Diagnose.}
\label{tab:observable_distributions}
\end{longtable}}
% }
%}
% \caption{Symptomverteilung \textit{TODO: ausführlicher formulieren}}
% \label{tab:results:observable_distributions}
% \end{table}

==> chapters/tables/WrongClassificationProbsPretty_EP.tex <==
{\renewcommand{\arraystretch}{1.1}
\scriptsize
\begin{longtable}{lllllllll}
\multicolumn{9}{c}{Diagnosewahrscheinlichkeiten der falsch klassifizierten Beispiele} \\ \hline
Alg. & Erwartete Diagnose & wahrsch. Diagnose & BT & CHA & MA & MO & THA & $\Delta$ \\ \hline \endhead
EP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0 & 100 & 0 & 100 \\
EP & MigraineWithAura & MigraineWithoutAura & 6,7 & 0,1 & 0,1 & 100 & 0 & 99,9 \\
EP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 0,1 & 100 & 0,2 & 99,9 \\
EP & MigraineWithAura & MigraineWithoutAura & 6,7 & 0 & 0 & 100 & 0 & 100 \\
EP & MigraineWithAura & MigraineWithoutAura & 0,7 & 0 & 0 & 100 & 0 & 100 \\
EP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 0,1 & 100 & 0 & 99,9 \\
EP & MigraineWithAura & MigraineWithoutAura & 6,7 & 0 & 0,7 & 100 & 0,3 & 99,3 \\
EP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 0,3 & 100 & 0 & 99,7 \\
EP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0,1 & 100 & 0 & 99,9 \\
EP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0,3 & 100 & 0,2 & 99,7 \\
EP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0,3 & 100 & 0,1 & 99,7 \\
EP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 0 & 100 & 0 & 100 \\
EP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0,1 & 100 & 0 & 99,9 \\
EP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 0,1 & 100 & 0 & 99,9 \\
EP & MigraineWithoutAura & MigraineWithAura & 1,5 & 0 & 100 & 7,4 & 0 & 92,6 \\
EP & MigraineWithoutAura & MigraineWithAura & 53,5 & 0 & 100 & 6 & 6,2 & 94 \\
EP & TensionHeadache & BrainTumor & 1,9 & 0 & 0 & 0 & 1,1 & 0,9 \\
EP & TensionHeadache & MigraineWithoutAura & 58,5 & 0 & 0 & 100 & 0,1 & 99,9 \\ \hline
JTBP & ClusterHeadache & BrainTumor & 1,9 & 0 & 0 & 0 & 0 & 1,9 \\
JTBP & ClusterHeadache & BrainTumor & 35,6 & 2,8 & 0 & 0 & 0 & 32,8 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 11,8 & 88,2 & 0 & 76,4 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 8,7 & 1,5 & 1,1 & 97,5 & 0 & 96,5 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 1,1 & 0 & 2,2 & 98 & 0,1 & 95,8 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 8,7 & 0 & 10,7 & 89,3 & 0 & 78,6 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 3,5 & 0 & 24,3 & 75,7 & 0,1 & 51,4 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 1,1 & 0 & 2 & 98,1 & 0 & 96 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 8,7 & 0 & 2,3 & 98,5 & 0,1 & 96,2 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 1,1 & 0 & 2,3 & 98 & 0 & 95,7 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 7,5 & 92,6 & 0 & 85,2 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 1 & 99,2 & 0,1 & 98,2 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 6,1 & 94,2 & 0,1 & 88,1 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 1,1 & 0 & 10,7 & 89,3 & 0 & 78,6 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 7,5 & 92,6 & 0 & 85,2 \\
JTBP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 7,1 & 92,9 & 0 & 85,8 \\
JTBP & MigraineWithoutAura & MigraineWithAura & 2 & 0 & 99,2 & 8,2 & 0 & 91 \\
JTBP & MigraineWithoutAura & MigraineWithAura & 60,3 & 0 & 98,9 & 7,3 & 1,5 & 91,7 \\
JTBP & TensionHeadache & BrainTumor & 0,7 & 0 & 0 & 0 & 0,3 & 0,4 \\
JTBP & TensionHeadache & BrainTumor & 1,9 & 0 & 0 & 0 & 1,4 & 0,5 \\
JTBP & TensionHeadache & BrainTumor & 5 & 0 & 0 & 0 & 0,6 & 4,4 \\
JTBP & TensionHeadache & MigraineWithoutAura & 60,1 & 0 & 15,4 & 61,7 & 22,9 & 38,9 \\ \hline
VMP & MigraineWithAura & ClusterHeadache & 58,7 & 100 & 17,8 & 0,1 & 99,6 & 82,2 \\
VMP & MigraineWithAura & ClusterHeadache & 6,7 & 100 & 0,1 & 4,4 & 0 & 99,9 \\
VMP & MigraineWithAura & ClusterHeadache & 0,2 & 100 & 29,6 & 3,3 & 0 & 70,4 \\
VMP & MigraineWithAura & ClusterHeadache & 0,7 & 100 & 20,4 & 3,6 & 99,6 & 79,6 \\
VMP & MigraineWithAura & ClusterHeadache & 1,8 & 100 & 3,1 & 0,1 & 100 & 96,9 \\
VMP & MigraineWithAura & ClusterHeadache & 6,7 & 100 & 3,7 & 0,1 & 99,9 & 96,3 \\
VMP & MigraineWithAura & ClusterHeadache & 1,8 & 100 & 15,6 & 0,6 & 0,1 & 84,4 \\
VMP & MigraineWithAura & ClusterHeadache & 1,8 & 100 & 25,7 & 0,9 & 0,1 & 74,3 \\
VMP & MigraineWithAura & ClusterHeadache & 53,5 & 100 & 0,2 & 0 & 0 & 99,8 \\
VMP & MigraineWithAura & ClusterHeadache & 1,5 & 100 & 1,3 & 0,2 & 100 & 98,7 \\
VMP & MigraineWithAura & ClusterHeadache & 53,8 & 100 & 14,5 & 1,9 & 99,7 & 85,5 \\
VMP & MigraineWithAura & ClusterHeadache & 0,4 & 100 & 0,7 & 5,6 & 99,9 & 99,3 \\
VMP & MigraineWithAura & ClusterHeadache & 6,8 & 100 & 17,1 & 0,1 & 99,7 & 82,9 \\
VMP & MigraineWithAura & ClusterHeadache & 1,8 & 100 & 1,4 & 0,2 & 0 & 98,6 \\
VMP & MigraineWithAura & ClusterHeadache & 1,5 & 100 & 17 & 2,5 & 99,9 & 83 \\
VMP & MigraineWithAura & ClusterHeadache & 0,2 & 100 & 1 & 0 & 100 & 99 \\
VMP & MigraineWithAura & MigraineWithoutAura & 24,9 & 0 & 77,6 & 100 & 0 & 22,4 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0 & 100 & 0 & 100 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 81,1 & 100 & 0 & 18,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 80 & 100 & 0,3 & 20 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 78,7 & 100 & 0,4 & 21,3 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 81,1 & 100 & 0,4 & 18,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,7 & 0 & 78,7 & 100 & 0,1 & 21,3 \\
VMP & MigraineWithAura & MigraineWithoutAura & 53,5 & 0 & 41,3 & 100 & 0 & 58,7 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 29 & 100 & 0 & 71 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 86,3 & 100 & 0,8 & 13,7 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 56,4 & 100 & 0,1 & 43,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 6,7 & 0 & 0 & 100 & 0 & 100 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 59 & 100 & 0,1 & 41 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 62,5 & 100 & 0 & 37,5 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 62,5 & 100 & 0 & 37,5 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 81,1 & 100 & 0 & 18,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 76,2 & 100 & 0 & 23,8 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,7 & 0 & 81,1 & 100 & 0 & 18,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 81,1 & 100 & 0,2 & 18,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 22,9 & 100 & 0 & 77,1 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 29 & 100 & 0 & 71 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,7 & 0 & 12 & 100 & 0 & 88 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 52,8 & 100 & 0 & 47,2 \\
VMP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 44,9 & 100 & 0 & 55,1 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 0,1 & 100 & 0 & 99,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 17,6 & 100 & 0 & 82,4 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 80,7 & 100 & 0,1 & 19,3 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 37,3 & 100 & 0,2 & 62,7 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 76,2 & 100 & 0 & 23,8 \\
VMP & MigraineWithAura & MigraineWithoutAura & 6,7 & 0 & 64,7 & 100 & 0 & 35,3 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 54,9 & 100 & 0 & 45,1 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 81,1 & 100 & 0 & 18,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,7 & 0 & 71,7 & 100 & 0,1 & 28,3 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 81,1 & 100 & 0 & 18,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 61 & 100 & 0 & 39 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 68,6 & 100 & 0 & 31,4 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 82,4 & 100 & 28,2 & 17,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 37,8 & 100 & 0,5 & 62,2 \\
VMP & MigraineWithAura & MigraineWithoutAura & 6,7 & 0 & 0,6 & 100 & 0,5 & 99,4 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 78,7 & 100 & 0,1 & 21,3 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 0,3 & 100 & 0,1 & 99,7 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 60,8 & 100 & 1,4 & 39,2 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 81,5 & 100 & 23,1 & 18,5 \\
VMP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 44,9 & 100 & 0 & 55,1 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 74,8 & 100 & 0,4 & 25,2 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 52,8 & 100 & 0 & 47,2 \\
VMP & MigraineWithAura & MigraineWithoutAura & 87 & 0 & 52,8 & 100 & 0 & 47,2 \\
VMP & MigraineWithAura & MigraineWithoutAura & 10,7 & 0 & 61 & 100 & 0 & 39 \\
VMP & MigraineWithAura & MigraineWithoutAura & 58,5 & 0 & 86,6 & 100 & 0,2 & 13,4 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 39,8 & 100 & 0,6 & 60,2 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 82,4 & 100 & 0,8 & 17,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 69 & 100 & 0,2 & 31 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0,1 & 100 & 0 & 99,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 61 & 100 & 0 & 39 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 62,5 & 100 & 0 & 37,5 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,7 & 0 & 78,7 & 100 & 0,1 & 21,3 \\
VMP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 81,1 & 100 & 0,1 & 18,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 56,4 & 100 & 0 & 43,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0,3 & 100 & 0,2 & 99,7 \\
VMP & MigraineWithAura & MigraineWithoutAura & 24,9 & 0 & 81,1 & 100 & 0 & 18,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 84,7 & 100 & 3,3 & 15,3 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 22,9 & 100 & 0 & 77,1 \\
VMP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 62,5 & 100 & 0 & 37,5 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 82,4 & 100 & 0,1 & 17,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 82,4 & 100 & 3,6 & 17,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0,3 & 100 & 0,1 & 99,7 \\
VMP & MigraineWithAura & MigraineWithoutAura & 10,7 & 0 & 58,9 & 100 & 0,6 & 41,1 \\
VMP & MigraineWithAura & MigraineWithoutAura & 6,7 & 0 & 35,4 & 100 & 0 & 64,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 6,7 & 0 & 78,7 & 100 & 0,1 & 21,3 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,7 & 0 & 61 & 100 & 0 & 39 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 65,9 & 100 & 0,1 & 34,1 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 35,4 & 100 & 0 & 64,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 58,5 & 0 & 85,2 & 100 & 25,5 & 14,8 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 0,1 & 100 & 0 & 99,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 6,7 & 0 & 35,4 & 100 & 0 & 64,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 2 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 82,4 & 100 & 1,5 & 17,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,4 & 0 & 79,8 & 100 & 0,1 & 20,2 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 77,6 & 100 & 0 & 22,4 \\
VMP & MigraineWithAura & MigraineWithoutAura & 10,7 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 64,5 & 100 & 0 & 35,5 \\
VMP & MigraineWithAura & MigraineWithoutAura & 53,5 & 0 & 37,3 & 100 & 0,1 & 62,7 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,7 & 0 & 60,9 & 100 & 0,3 & 39,1 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 61 & 100 & 0,1 & 39 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 61 & 100 & 0 & 39 \\
VMP & MigraineWithAura & MigraineWithoutAura & 53,5 & 0 & 76,2 & 100 & 0 & 23,8 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 44,9 & 100 & 0 & 55,1 \\
VMP & MigraineWithAura & MigraineWithoutAura & 8,1 & 0 & 62,5 & 100 & 0 & 37,5 \\
VMP & MigraineWithAura & MigraineWithoutAura & 0,2 & 0 & 79,8 & 100 & 0,1 & 20,2 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 81,2 & 100 & 0,2 & 18,8 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,5 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & MigraineWithoutAura & 1,8 & 0 & 35,4 & 100 & 0 & 64,6 \\
VMP & MigraineWithAura & MigraineWithoutAura & 53,5 & 0 & 76,1 & 100 & 0 & 23,9 \\
VMP & MigraineWithAura & TensionHeadache & 25,3 & 100 & 39,4 & 0,7 & 100 & 60,6 \\
VMP & MigraineWithAura & TensionHeadache & 1,4 & 0 & 0 & 0 & 100 & 100 \\
VMP & MigraineWithAura & TensionHeadache & 0,4 & 100 & 0,2 & 2,5 & 100 & 99,8 \\
VMP & MigraineWithAura & TensionHeadache & 1,8 & 100 & 27,3 & 0,2 & 100 & 72,7 \\
VMP & MigraineWithAura & TensionHeadache & 0,7 & 0 & 1 & 3,2 & 100 & 99 \\
VMP & MigraineWithAura & TensionHeadache & 58,9 & 100 & 40,4 & 0,8 & 100 & 59,6 \\
VMP & MigraineWithAura & TensionHeadache & 58,8 & 100 & 32,5 & 3,9 & 100 & 67,5 \\
VMP & MigraineWithAura & TensionHeadache & 1,8 & 99,7 & 1 & 0 & 100 & 99 \\
VMP & MigraineWithAura & TensionHeadache & 1,8 & 100 & 0,1 & 0,8 & 100 & 99,9 \\
VMP & MigraineWithoutAura & ClusterHeadache & 1,8 & 100 & 0,1 & 3,2 & 100 & 96,8 \\
VMP & MigraineWithoutAura & MigraineWithAura & 1,5 & 0 & 100 & 7,4 & 0 & 92,6 \\
VMP & MigraineWithoutAura & TensionHeadache & 0,2 & 99,9 & 0,5 & 4,5 & 100 & 95,5 \\
VMP & MigraineWithoutAura & TensionHeadache & 1,8 & 100 & 1 & 9,3 & 100 & 90,7 \\
VMP & MigraineWithoutAura & TensionHeadache & 24,9 & 100 & 0,1 & 2,3 & 100 & 97,7 \\
VMP & MigraineWithoutAura & TensionHeadache & 0,2 & 99,5 & 0,3 & 11,7 & 100 & 88,3 \\
VMP & MigraineWithoutAura & TensionHeadache & 1,5 & 100 & 0,1 & 2,3 & 100 & 97,7 \\
VMP & MigraineWithoutAura & TensionHeadache & 2 & 99,8 & 0,2 & 3,2 & 99,9 & 96,7 \\
VMP & MigraineWithoutAura & TensionHeadache & 1,5 & 100 & 0,2 & 0,9 & 100 & 99 \\
VMP & MigraineWithoutAura & TensionHeadache & 53,6 & 100 & 0,2 & 2,2 & 100 & 97,8 \\
VMP & MigraineWithoutAura & TensionHeadache & 1,8 & 99,5 & 0,2 & 8,3 & 100 & 91,7 \\
VMP & MigraineWithoutAura & TensionHeadache & 0,2 & 100 & 0,2 & 3,9 & 100 & 96,1 \\
VMP & MigraineWithoutAura & TensionHeadache & 1,8 & 99,7 & 0,2 & 9,9 & 100 & 90,1 \\
VMP & TensionHeadache & BrainTumor & 1,9 & 0 & 0 & 0 & 1,1 & 0,9 \\
VMP & TensionHeadache & ClusterHeadache & 8,1 & 100 & 0 & 0 & 9 & 91 \\ \hline
\caption{Diagnosewahrscheinlichkeiten für falsch klassifizierte Beispiele. Die wahrscheinlichste Diagnose wurde fett, die erwartete kursiv markiert.}
\label{tab:results:wrong_classification_diagnose_probs}
\end{longtable}}
